Improved Dynamical Constraints on the Mass of the central Black Hole in NGC 404

We explore the nucleus of the nearby 10$^9M_{\odot}$~early-type galaxy (ETGs), NGC~404, using Hubble Space Telescope (HST)/STIS spectroscopy and WFC3 imaging. We first present evidence for nuclear variability in UV, optical, and infrared filters over a time period of 15~years. This variability adds to the already substantial evidence for an accreting black hole at the center of NGC~404. We then redetermine the dynamical black hole mass in NGC~404 including modeling of the nuclear stellar populations. We combine HST/STIS spectroscopy with WFC3 images to create a local color-$M/L$~relation derived from stellar population modeling of the STIS data. We then use this to create a mass model for the nuclear region. We use Jeans modeling to fit this mass model to adaptive optics (AO) stellar kinematic observations from Gemini/NIFS. From our stellar dynamical modeling, we find a 3$\sigma$ upper limit on the black hole mass of $1.5\times10^5M_{\odot}$. Given the accretion evidence for a black hole, this upper limit makes NGC~404 the lowest mass central black hole with dynamical mass constraints. We find that the kinematics of H$_2$ emission line gas show evidence for non-gravitational motions preventing the use of gas dynamical modeling to constrain the black hole mass. Our stellar population modeling also reveals that the central, counter-rotating region of the nuclear cluster is dominated by $\sim$1~Gyr old populations.

==> ngc404.tex <==

@ARTICLE{Spiniello14,
   author = {{Spiniello}, C. and {Trager}, S. and {Koopmans}, L.~V.~E. and 
	{Conroy}, C.},
    title = "{The stellar IMF in early-type galaxies from a non-degenerate set of optical line indices}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1305.2873},
 keywords = {gravitational lensing: strong, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: kinematics and dynamics, galaxies: structure, dark matter},
     year = 2014,
    month = feb,
   volume = 438,
    pages = {1483-1499},
      doi = {10.1093/mnras/stt2282},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.1483S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Scott13a,
   author = {{Scott}, N. and {Graham}, A.~W.},
    title = "{Updated Mass Scaling Relations for Nuclear Star Clusters and a Comparison to Supermassive Black Holes}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1205.5338},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: fundamental parameters, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: star clusters: general, galaxies: structure },
     year = 2013,
    month = feb,
   volume = 763,
      eid = {76},
    pages = {76},
      doi = {10.1088/0004-637X/763/2/76},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...763...76S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Seth08b,
   author = {{Seth}, A.~C. and {Blum}, R.~D. and {Bastian}, N. and {Caldwell}, N. and 
	{Debattista}, V.~P.},
    title = "{The Rotating Nuclear Star Cluster in NGC 4244}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0807.3044},
 keywords = {Galaxies: Formation, Galaxies: Individual: NGC Number: NGC 4244, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Spiral, Galaxies: Star Clusters},
     year = 2008,
    month = nov,
   volume = 687,
    pages = {997-1003},
      doi = {10.1086/591935},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...687..997S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Seth08a,
   author = {{Seth}, A. and {Ag{\"u}eros}, M. and {Lee}, D. and {Basu-Zych}, A.
	},
    title = "{The Coincidence of Nuclear Star Clusters and Active Galactic Nuclei}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0801.0439},
 keywords = {Galaxies: Active, Galaxies: Formation, Galaxies: Nuclei, Galaxies: Star Clusters},
     year = 2008,
    month = may,
   volume = 678,
    pages = {116-130},
      doi = {10.1086/528955},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...678..116S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Seth06,
   author = {{Seth}, A.~C. and {Dalcanton}, J.~J. and {Hodge}, P.~W. and 
	{Debattista}, V.~P.},
    title = "{Clues to Nuclear Star Cluster Formation from Edge-on Spirals}",
  journal = {\aj},
   eprint = {astro-ph/0609302},
 keywords = {Galaxies: Formation, galaxies: individual (IC 5052), Galaxies: Individual: NGC Number: NGC 4244, galaxies: individual (NGC 4206), Galaxies: Nuclei, Galaxies: Spiral, Galaxies: Star Clusters},
     year = 2006,
    month = dec,
   volume = 132,
    pages = {2539-2555},
      doi = {10.1086/508994},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....132.2539S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Seth10,
   author = {{Seth}, A.~C. and {Cappellari}, M. and {Neumayer}, N. and {Caldwell}, N. and 
	{Bastian}, N. and {Olsen}, K. and {Blum}, R.~D. and {Debattista}, V.~P. and 
\citep{}	{McDermid}, R. and {Puzia}, T. and {Stephens}, A.},
    title = "{The NGC 404 Nucleus: Star Cluster and Possible Intermediate-mass Black Hole}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1003.0680},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: formation, galaxies: individual: NGC 404, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: structure},
     year = 2010,
    month = may,
   volume = 714,
    pages = {713-731},
      doi = {10.1088/0004-637X/714/1/713},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714..713S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Graham08,
   author = {{Graham}, A.~W.},
    title = "{Populating the Galaxy Velocity Dispersion - Supermassive Black Hole Mass Diagram: A Catalogue of (M$_{bh}$, {$\sigma$}) Values}",
  journal = {\pasa},
archivePrefix = "arXiv",
   eprint = {0807.2549},
 keywords = {catalogues, black hole physics, galaxies: bulges, galaxies: fundamental parameters, galaxies: kinematics and dynamics, galaxies: nuclei,},
     year = 2008,
    month = nov,
   volume = 25,
    pages = {167-175},
      doi = {10.1071/AS08013},
   adsurl = {http://adsabs.harvard.edu/abs/2008PASA...25..167G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gultekin09,
   author = {{G{\"u}ltekin}, K. and {Richstone}, D.~O. and {Gebhardt}, K. and 
	{Lauer}, T.~R. and {Tremaine}, S. and {Aller}, M.~C. and {Bender}, R. and 
	{Dressler}, A. and {Faber}, S.~M. and {Filippenko}, A.~V. and 
	{Green}, R. and {Ho}, L.~C. and {Kormendy}, J. and {Magorrian}, J. and 
	{Pinkney}, J. and {Siopis}, C.},
    title = "{The M-{$\sigma$} and M-L Relations in Galactic Bulges, and Determinations of Their Intrinsic Scatter}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0903.4897},
 primaryClass = "astro-ph.GA",
 keywords = {black hole physics, galaxies: general, galaxies: nuclei, galaxies: statistics, stellar dynamics},
     year = 2009,
    month = jun,
   volume = 698,
    pages = {198-221},
      doi = {10.1088/0004-637X/698/1/198},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...698..198G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Charlot00,
   author = {{Charlot}, S. and {Fall}, S.~M.},
    title = "{A Simple Model for the Absorption of Starlight by Dust in Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/0003128},
 keywords = {ISM: Dust, Extinction, Galaxies: ISM, Galaxies: Starburst, Infrared: Galaxies, Ultraviolet: Galaxies},
     year = 2000,
    month = aug,
   volume = 539,
    pages = {718-731},
      doi = {10.1086/309250},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...539..718C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{prop12611hst,
   author = {{Seth}, A.},
    title = "{Weighing the Low Mass Central Black Hole in NGC404}",
howpublished = {HST Proposal},
     year = 2011,
    month = oct,
    pages = {12611},
   adsurl = {http://adsabs.harvard.edu/abs/2011hst..prop12611S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Krist11,
   author = {{Krist}, J.~E. and {Hook}, R.~N. and {Stoehr}, F.},
    title = "{20 years of Hubble Space Telescope optical modeling using Tiny Tim}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2011,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 8127,
    month = oct,
      eid = {81270J},
    pages = {0},
      doi = {10.1117/12.892762},
   adsurl = {http://adsabs.harvard.edu/abs/2011SPIE.8127E..0JK},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krajnovic09,
   author = {{Krajnovi{\'c}}, D. and {McDermid}, R.~M. and {Cappellari}, M. and 
	{Davies}, R.~L.},
    title = "{Determination of masses of the central black holes in NGC 524 and 2549 using laser guide star adaptive optics}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0907.3748},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: elliptical and lenticular, cD , galaxies: individual: NGC 524 , galaxies: individual: NGC 2549 , galaxies: kinematics and dynamics},
     year = 2009,
    month = nov,
   volume = 399,
    pages = {1839-1857},
      doi = {10.1111/j.1365-2966.2009.15415.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.399.1839K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Avila12,
   author = {{Avila}, R.~J. and {Hack}, W.~J. and {STScI AstroDrizzle Team}
	},
    title = "{AstroDrizzle: Aligning Images From Multiple Instruments}",
booktitle = {American Astronomical Society Meeting Abstracts 220},
     year = 2012,
   series = {American Astronomical Society Meeting Abstracts},
   volume = 220,
    month = may,
    pages = {\#135.13},
   adsurl = {http://adsabs.harvard.edu/abs/2012AAS...22013513A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Peng10,
   author = {{Peng}, C.~Y. and {Ho}, L.~C. and {Impey}, C.~D. and {Rix}, H.-W.
	},
    title = "{Detailed Decomposition of Galaxy Images. II. Beyond Axisymmetric Models}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0912.0731},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: bulges, galaxies: fundamental parameters, galaxies: structure, techniques: image processing, techniques: photometric},
     year = 2010,
    month = jun,
   volume = 139,
    pages = {2097-2129},
      doi = {10.1088/0004-6256/139/6/2097},
   adsurl = {http://adsabs.harvard.edu/abs/2010AJ....139.2097P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bruzual03,
   author = {{Bruzual}, G. and {Charlot}, S.},
    title = "{Stellar population synthesis at the resolution of 2003}",
  journal = {\mnras},
   eprint = {astro-ph/0309134},
 keywords = {stars: evolution, galaxies: evolution, galaxies: formation, galaxies: stellar content},
     year = 2003,
    month = oct,
   volume = 344,
    pages = {1000-1028},
      doi = {10.1046/j.1365-8711.2003.06897.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.344.1000B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Peng02,
   author = {{Peng}, C.~Y. and {Ho}, L.~C. and {Impey}, C.~D. and {Rix}, H.-W.
	},
    title = "{Detailed Structural Decomposition of Galaxy Images}",
  journal = {\aj},
   eprint = {astro-ph/0204182},
 keywords = {Galaxies: Bulges, Galaxies: Fundamental Parameters, Galaxies: Nuclei, Galaxies: Structure, Techniques: Image Processing, Techniques: Photometric},
     year = 2002,
    month = jul,
   volume = 124,
    pages = {266-293},
      doi = {10.1086/340952},
   adsurl = {http://adsabs.harvard.edu/abs/2002AJ....124..266P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bouchard10,
   author = {{Bouchard}, A. and {Prugniel}, P. and {Koleva}, M. and {Sharina}, M.
	},
    title = "{Stellar population and kinematics of NGC 404}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1001.4087},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: abundances, galaxies: dwarf, galaxies: evolution, galaxies: stellar content, techniques: spectroscopic},
     year = 2010,
    month = apr,
   volume = 513,
      eid = {A54},
    pages = {A54},
      doi = {10.1051/0004-6361/200913137},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...513A..54B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CidFernandes04,
   author = {{Cid Fernandes}, R. and {Gonz{\'a}lez Delgado}, R.~M. and {Schmitt}, H. and 
	{Storchi-Bergmann}, T. and {Martins}, L.~P. and {P{\'e}rez}, E. and 
	{Heckman}, T. and {Leitherer}, C. and {Schaerer}, D.},
    title = "{The Stellar Populations of Low-Luminosity Active Galactic Nuclei. I. Ground-based Observations}",
  journal = {\apj},
   eprint = {astro-ph/0401416},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Starburst, Galaxies: Stellar Content},
     year = 2004,
    month = apr,
   volume = 605,
    pages = {105-126},
      doi = {10.1086/382217},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...605..105C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bertelli94,
   author = {{Bertelli}, G. and {Bressan}, A. and {Chiosi}, C. and {Fagotto}, F. and 
	{Nasi}, E.},
    title = "{Theoretical isochrones from models with new radiative opacities}",
  journal = {\aaps},
 keywords = {STARS: EVOLUTION, INTERIORS, FUNDAMENTAL PARAMETERS, HR DIAGRAM},
     year = 1994,
    month = aug,
   volume = 106,
    pages = {275-302},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26AS..106..275B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Girardi00,
   author = {{Girardi}, L. and {Bressan}, A. and {Bertelli}, G. and {Chiosi}, C.
	},
    title = "{Evolutionary tracks and isochrones for low- and intermediate-mass stars: From 0.15 to 7 M$_{sun}$, and from Z=0.0004 to 0.03}",
  journal = {\aaps},
   eprint = {astro-ph/9910164},
 keywords = {STARS: EVOLUTION, STARS: INTERIORS, STARS: HERTZSPRUNG-RUSSELL (HR) DIAGRAM, STARS: LOW-MASS},
     year = 2000,
    month = feb,
   volume = 141,
    pages = {371-383},
      doi = {10.1051/aas:2000126},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26AS..141..371G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LeBorgne03,
   author = {{Le Borgne}, J.-F. and {Bruzual}, G. and {Pell{\'o}}, R. and 
	{Lan{\c c}on}, A. and {Rocca-Volmerange}, B. and {Sanahuja}, B. and 
	{Schaerer}, D. and {Soubiran}, C. and {V{\'{\i}}lchez-G{\'o}mez}, R.
	},
    title = "{STELIB: A library of stellar spectra at R \~{} 2000}",
  journal = {\aap},
   eprint = {astro-ph/0302334},
 keywords = {atlases, stars: fundamental parameters, galaxies: stellar content.},
     year = 2003,
    month = may,
   volume = 402,
    pages = {433-442},
      doi = {10.1051/0004-6361:20030243},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...402..433L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marigo07,
   author = {{Marigo}, P. and {Girardi}, L.},
    title = "{Evolution of asymptotic giant branch stars. I. Updated synthetic TP-AGB models and their basic calibration}",
  journal = {\aap},
   eprint = {astro-ph/0703139},
 keywords = {stars: AGB and post-AGB, stars: carbon, stars: mass-loss, stars: general, stars: evolution, stars: abundances},
     year = 2007,
    month = jul,
   volume = 469,
    pages = {239-263},
      doi = {10.1051/0004-6361:20066772},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..239M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marigo08,
   author = {{Marigo}, P. and {Girardi}, L. and {Bressan}, A. and {Groenewegen}, M.~A.~T. and 
	{Silva}, L. and {Granato}, G.~L.},
    title = "{Evolution of asymptotic giant branch stars. II. Optical to far-infrared isochrones with improved TP-AGB models}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0711.4922},
 keywords = {astronomical data bases: miscellaneous, stars: AGB and post-AGB, stars: carbon, stars: evolution, galaxies: Magellanic Clouds, stars: Hertzsprung-Russell (HR) and C-M diagrams},
     year = 2008,
    month = may,
   volume = 482,
    pages = {883-905},
      doi = {10.1051/0004-6361:20078467},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...482..883M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tremonti04,
   author = {{Tremonti}, C.~A. and {Heckman}, T.~M. and {Kauffmann}, G. and 
	{Brinchmann}, J. and {Charlot}, S. and {White}, S.~D.~M. and 
	{Seibert}, M. and {Peng}, E.~W. and {Schlegel}, D.~J. and {Uomoto}, A. and 
	{Fukugita}, M. and {Brinkmann}, J.},
    title = "{The Origin of the Mass-Metallicity Relation: Insights from 53,000 Star-forming Galaxies in the Sloan Digital Sky Survey}",
  journal = {\apj},
   eprint = {astro-ph/0405537},
 keywords = {Galaxies: Abundances, Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: Statistics},
     year = 2004,
    month = oct,
   volume = 613,
    pages = {898-913},
      doi = {10.1086/423264},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...613..898T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Koleva08,
   author = {{Koleva}, M. and {Prugniel}, P. and {Ocvirk}, P. and {Le Borgne}, D. and 
	{Soubiran}, C.},
    title = "{Spectroscopic ages and metallicities of stellar populations: validation of full spectrum fitting}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0801.0871},
 keywords = {techniques: spectroscopic , globular clusters: general , Galaxy: stellar content},
     year = 2008,
    month = apr,
   volume = 385,
    pages = {1998-2010},
      doi = {10.1111/j.1365-2966.2008.12908.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385.1998K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wallace96,
   author = {{Wallace}, L. and {Hinkle}, K.},
    title = "{High-Resolution Spectra of Ordinary Cool Stars in the K Band}",
  journal = {\apjs},
 keywords = {ATLASES, INFRARED: STARS, LINE: IDENTIFICATION, STARS: LATE-TYPE},
     year = 1996,
    month = nov,
   volume = 107,
    pages = {312},
      doi = {10.1086/192367},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJS..107..312W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Walcher06,
   author = {{Walcher}, C.~J. and {B{\"o}ker}, T. and {Charlot}, S. and {Ho}, L.~C. and 
	{Rix}, H.-W. and {Rossa}, J. and {Shields}, J.~C. and {van der Marel}, R.~P.
	},
    title = "{Stellar Populations in the Nuclei of Late-Type Spiral Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/0604138},
 keywords = {Galaxies: Nuclei, Galaxies: Spiral, Galaxies: Star Clusters, Galaxies: Structure},
     year = 2006,
    month = oct,
   volume = 649,
    pages = {692-708},
      doi = {10.1086/505166},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...649..692W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Siegel07,
   author = {{Siegel}, M.~H. and {Dotter}, A. and {Majewski}, S.~R. and {Sarajedini}, A. and 
	{Chaboyer}, B. and {Nidever}, D.~L. and {Anderson}, J. and {Mar{\'{\i}}n-Franch}, A. and 
	{Rosenberg}, A. and {Bedin}, L.~R. and {Aparicio}, A. and {King}, I. and 
	{Piotto}, G. and {Reid}, I.~N.},
    title = "{The ACS Survey of Galactic Globular Clusters: M54 and Young Populations in the Sagittarius Dwarf Spheroidal Galaxy}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0708.0027},
 keywords = {Galaxies: Individual: Name: Sagittarius, Galaxies: Star Clusters, Galaxies: Stellar Content, Galaxy: Globular Clusters: Individual: Messier Number: M54},
     year = 2007,
    month = sep,
   volume = 667,
    pages = {L57-L60},
      doi = {10.1086/522003},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...667L..57S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schlegel98,
   author = {{Schlegel}, D.~J. and {Finkbeiner}, D.~P. and {Davis}, M.},
    title = "{Maps of Dust Infrared Emission for Use in Estimation of Reddening and Cosmic Microwave Background Radiation Foregrounds}",
  journal = {\apj},
   eprint = {astro-ph/9710327},
 keywords = {COSMOLOGY: DIFFUSE RADIATION, COSMOLOGY: COSMIC MICROWAVE BACKGROUND, ISM: DUST, EXTINCTION, INTERPLANETARY MEDIUM, INFRARED: ISM: CONTINUUM, Cosmology: Cosmic Microwave Background, Cosmology: Diffuse Radiation, ISM: Dust, Extinction, Infrared: ISM: Continuum, Interplanetary Medium},
     year = 1998,
    month = jun,
   volume = 500,
    pages = {525-553},
      doi = {10.1086/305772},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...500..525S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Neumayer07,
   author = {{Neumayer}, N. and {Cappellari}, M. and {Reunanen}, J. and {Rix}, H.-W. and 
	{van der Werf}, P.~P. and {de Zeeuw}, P.~T. and {Davies}, R.~I.
	},
    title = "{The Central Parsecs of Centaurus A: High-excitation Gas, a Molecular Disk, and the Mass of the Black Hole}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0709.1877},
 keywords = {Galaxies: Individual: NGC Number: NGC 5128, Galaxies: Kinematics and Dynamics, Galaxies: Structure, Techniques: Spectroscopic},
     year = 2007,
    month = dec,
   volume = 671,
    pages = {1329-1344},
      doi = {10.1086/523039},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...671.1329N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{delrio04,
   author = {{del R{\'{\i}}o}, M.~S. and {Brinks}, E. and {Cepa}, J.},
    title = "{High-Resolution H I Observations of the Galaxy NGC 404: A Dwarf S0 with Abundant Interstellar Gas}",
  journal = {\aj},
   eprint = {astro-ph/0403467},
 keywords = {Galaxies: Elliptical and Lenticular, cD, galaxies: individual (NGC 404), Galaxies: Kinematics and Dynamics, Galaxies: Structure, Radio Lines: Galaxies},
     year = 2004,
    month = jul,
   volume = 128,
    pages = {89-102},
      doi = {10.1086/421358},
   adsurl = {http://adsabs.harvard.edu/abs/2004AJ....128...89D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ho97,
   author = {{Ho}, L.~C. and {Filippenko}, A.~V. and {Sargent}, W.~L.~W.},
    title = "{A Search for ``Dwarf'' Seyfert Nuclei. III. Spectroscopic Parameters and Properties of the Host Galaxies}",
  journal = {\apjs},
   eprint = {astro-ph/9704107},
 keywords = {GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: ACTIVE, GALAXIES: NUCLEI, GALAXIES: SEYFERT, GALAXIES: ISM, Galaxies: Active, Galaxies: Fundamental Parameters, Galaxies: ISM, Galaxies: Nuclei, Galaxies: Seyfert},
     year = 1997,
    month = oct,
   volume = 112,
    pages = {315-390},
      doi = {10.1086/313041},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJS..112..315H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dudik05,
   author = {{Dudik}, R.~P. and {Satyapal}, S. and {Gliozzi}, M. and {Sambruna}, R.~M.
	},
    title = "{A Chandra Snapshot Survey of Infrared-bright LINERs: A Possible Link Between Star Formation, Active Galactic Nucleus Fueling, and Mass Accretion}",
  journal = {\apj},
   eprint = {astro-ph/0410305},
 keywords = {Galaxies: Active, Galaxies: Nuclei, X-Rays: Galaxies},
     year = 2005,
    month = feb,
   volume = 620,
    pages = {113-125},
      doi = {10.1086/426856},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...620..113D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ZhangWei09,
   author = {{Zhang}, W.~M. and {Soria}, R. and {Zhang}, S.~N. and {Swartz}, D.~A. and 
	{Liu}, J.~F.},
    title = "{A Census of X-ray Nuclear Activity in Nearby Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0904.1091},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: active, galaxies: nuclei, galaxies: statistics, X-rays: galaxies},
     year = 2009,
    month = jul,
   volume = 699,
    pages = {281-297},
      doi = {10.1088/0004-637X/699/1/281},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...699..281Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Paragi14,
   author = {{Paragi}, Z. and {Frey}, S. and {Kaaret}, P. and {Cseh}, D. and 
	{Overzier}, R. and {Kharb}, P.},
    title = "{Probing the Active Massive Black Hole Candidate in the Center of NGC 404 with VLBI}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1406.4752},
 keywords = {black hole physics, galaxies: active, galaxies: individual: NGC 404, radio continuum: galaxies, X-rays: galaxies},
     year = 2014,
    month = aug,
   volume = 791,
      eid = {2},
    pages = {2},
      doi = {10.1088/0004-637X/791/1/2},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...791....2P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nagar05,
   author = {{Nagar}, N.~M. and {Falcke}, H. and {Wilson}, A.~S.},
    title = "{Radio sources in low-luminosity active galactic nuclei. IV. Radio luminosity function, importance of jet power, and radio properties of the complete Palomar sample}",
  journal = {\aap},
   eprint = {astro-ph/0502551},
 keywords = {accretion, accretion disks, galaxies: jets, galaxies: nuclei, radio continuum: galaxies, surveys},
     year = 2005,
    month = may,
   volume = 435,
    pages = {521-543},
      doi = {10.1051/0004-6361:20042277},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...435..521N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nyland12,
   author = {{Nyland}, K. and {Marvil}, J. and {Wrobel}, J.~M. and {Young}, L.~M. and 
	{Zauderer}, B.~A.},
    title = "{The Intermediate-mass Black Hole Candidate in the Center of NGC 404: New Evidence from Radio Continuum Observations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1204.3089},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: active, galaxies: dwarf, galaxies: individual: NGC 404, galaxies: nuclei, galaxies: star formation, radio continuum: galaxies},
     year = 2012,
    month = jul,
   volume = 753,
      eid = {103},
    pages = {103},
      doi = {10.1088/0004-637X/753/2/103},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...753..103N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gonzalez06,
   author = {{Gonz{\'a}lez-Mart{\'{\i}}n}, O. and {Masegosa}, J. and {M{\'a}rquez}, I. and 
	{Guerrero}, M.~A. and {Dultzin-Hacyan}, D.},
    title = "{X-ray nature of the LINER nuclear sources}",
  journal = {\aap},
   eprint = {astro-ph/0605629},
 keywords = {galaxies: nuclei, X-rays: galaxies, galaxies: active},
     year = 2006,
    month = dec,
   volume = 460,
    pages = {45-57},
      doi = {10.1051/0004-6361:20054756},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...460...45G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Satyapal08,
   author = {{Satyapal}, S. and {Vega}, D. and {Dudik}, R.~P. and {Abel}, N.~P. and 
	{Heckman}, T.},
    title = "{Spitzer Uncovers Active Galactic Nuclei Missed by Optical Surveys in Seven Late-Type Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0801.2759},
 keywords = {Black Hole Physics, Cosmology: Dark Matter, Galaxies: Active, Galaxies: Spiral, Infrared: Galaxies},
     year = 2008,
    month = apr,
   volume = 677,
    pages = {926-942},
      doi = {10.1086/529014},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...677..926S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Satyapal04,
   author = {{Satyapal}, S. and {Sambruna}, R.~M. and {Dudik}, R.~P.},
    title = "{A joint mid-infrared spectroscopic and X-ray imaging investigation of LINER galaxies}",
  journal = {\aap},
   eprint = {astro-ph/0309082},
 keywords = {galaxies: starburst, X-rays: galaxies, infared: galaxies},
     year = 2004,
    month = feb,
   volume = 414,
    pages = {825-838},
      doi = {10.1051/0004-6361:20031609},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...414..825S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Satyapal09,
   author = {{Satyapal}, S. and {B{\"o}ker}, T. and {Mcalpine}, W. and {Gliozzi}, M. and 
	{Abel}, N.~P. and {Heckman}, T.},
    title = "{The Incidence of Active Galactic Nuclei in Pure Disk Galaxies: The Spitzer View}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0908.1820},
 primaryClass = "astro-ph.CO",
 keywords = {black hole physics, dark matter, galaxies: active, galaxies: spiral, infrared: galaxies},
     year = 2009,
    month = oct,
   volume = 704,
    pages = {439-452},
      doi = {10.1088/0004-637X/704/1/439},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...704..439S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maoz05,
   author = {{Maoz}, D. and {Nagar}, N.~M. and {Falcke}, H. and {Wilson}, A.~S.
	},
    title = "{The Murmur of the Sleeping Black Hole: Detection of Nuclear Ultraviolet Variability in LINER Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/0502347},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Starburst, Galaxies: Quasars: General, Ultraviolet: Galaxies},
     year = 2005,
    month = jun,
   volume = 625,
    pages = {699-715},
      doi = {10.1086/429795},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...625..699M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MaozEyal98,
   author = {{Maoz}, E.},
    title = "{Dynamical Constraints on Alternatives to Supermassive Black Holes in Galactic Nuclei}",
  journal = {\apjl},
   eprint = {astro-ph/9710309},
 keywords = {BLACK HOLE PHYSICS, GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: NUCLEI, Black Hole Physics, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei},
     year = 1998,
    month = feb,
   volume = 494,
    pages = {L181-L184},
      doi = {10.1086/311194},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...494L.181M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maoz98,
   author = {{Maoz}, D. and {Koratkar}, A. and {Shields}, J.~C. and {Ho}, L.~C. and 
	{Filippenko}, A.~V. and {Sternberg}, A.},
    title = "{The Ultraviolet Spectra of LINERs: A Comparative Study}",
  journal = {\aj},
   eprint = {astro-ph/9710323},
 keywords = {GALAXIES: ACTIVE, GALAXIES: NUCLEI, GALAXIES: STAR CLUSTERS, ULTRAVIOLET EMISSION},
     year = 1998,
    month = jul,
   volume = 116,
    pages = {55-67},
      doi = {10.1086/300403},
   adsurl = {http://adsabs.harvard.edu/abs/1998AJ....116...55M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Plana98,
   author = {{Plana}, H. and {Boulesteix}, J. and {Amram}, P. and {Carignan}, C. and 
	{Mendes de Oliveira}, C.},
    title = "{Extended ionized gas in elliptical galaxies. II. Velocity and monochromatic maps of 11 elliptical and lenticular galaxies}",
  journal = {\aaps},
 keywords = {GALAXIES: ELLIPTICAL AND LENTICULAR, KINEMATICS, ISM},
     year = 1998,
    month = feb,
   volume = 128,
    pages = {75-109},
      doi = {10.1051/aas:1998378},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26AS..128...75P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pogge00,
   author = {{Pogge}, R.~W. and {Maoz}, D. and {Ho}, L.~C. and {Eracleous}, M.
	},
    title = "{The Narrow-Line Regions of LINERS as Resolved with the Hubble Space Telescope}",
  journal = {\apj},
   eprint = {astro-ph/9910375},
 keywords = {GALAXIES: ACTIVE, GALAXIES: ISM, GALAXIES: NUCLEI, GALAXIES: SEYFERT},
     year = 2000,
    month = mar,
   volume = 532,
    pages = {323-339},
      doi = {10.1086/308567},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...532..323P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Binder11,
   author = {{Binder}, B. and {Williams}, B.~F. and {Eracleous}, M. and {Seth}, A.~C. and 
	{Dalcanton}, J.~J. and {Skillman}, E.~D. and {Weisz}, D.~R. and 
	{Anderson}, S.~F. and {Gaetz}, T.~J. and {Plucinsky}, P.~P.},
    title = "{A Deep Chandra View of the NGC 404 Central Engine}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1104.0981},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: active, galaxies: individual: NGC 404, galaxies: nuclei, X-rays: general},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {77},
    pages = {77},
      doi = {10.1088/0004-637X/737/2/77},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737...77B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lira00,
   author = {{Lira}, P. and {Lawrence}, A. and {Johnson}, R.~A.},
    title = "{Multiwavelength study of the nuclei of a volume-limited sample of galaxies - I. X-ray observations}",
  journal = {\mnras},
   eprint = {astro-ph/0005285},
 keywords = {GALAXIES: ACTIVE, GALAXIES: GENERAL, GALAXIES: NUCLEI, X-RAYS: GALAXIES},
     year = 2000,
    month = nov,
   volume = 319,
    pages = {17-42},
      doi = {10.1046/j.1365-8711.2000.03659.x},
   adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.319...17L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eracleous02,
   author = {{Eracleous}, M. and {Shields}, J.~C. and {Chartas}, G. and {Moran}, E.~C.
	},
    title = "{Three LINERs under the Chandra X-Ray Microscope}",
  journal = {\apj},
   eprint = {astro-ph/0109246},
 keywords = {Galaxies: Active, Galaxies: Nuclei, X-Rays: Binaries, X-Rays: Galaxies},
     year = 2002,
    month = jan,
   volume = 565,
    pages = {108-124},
      doi = {10.1086/324394},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...565..108E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Abel08,
   author = {{Abel}, N.~P. and {Satyapal}, S.},
    title = "{[Ne V] Emission in Optically Classified Starbursts}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0801.2766},
 keywords = {Galaxies: Active, Galaxies: Starburst, Infrared: Galaxies, Line: Formation},
     year = 2008,
    month = may,
   volume = 678,
    pages = {686-692},
      doi = {10.1086/529013},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...678..686A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Emsellem94b,
   author = {{Emsellem}, E. and {Monnet}, G. and {Bacon}, R. and {Nieto}, J.-L.
	},
    title = "{The multi-gaussian expansion method: a tool for building realistic photometric and kinematical models of stellar systems II. Application to the central region of the Sombrero Galaxy (NGC 4594)}",
  journal = {\aap},
 keywords = {GALAXIES: INDIVIDUAL: NGC 4594, GALAXIES: STRUCTURE, GALAXIES: LUMINOSITY FUNCTION, MASS FUNCTION, GALAXIES: KINEMATICS AND DYNAMICS OF, GALAXIES: NUCLEI, IMAGE PROCESSING},
     year = 1994,
    month = may,
   volume = 285,
    pages = {739-750},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...285..739E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari02,
   author = {{Cappellari}, M.},
    title = "{Efficient multi-Gaussian expansion of galaxies}",
  journal = {\mnras},
   eprint = {astro-ph/0201430},
 keywords = {stellar dynamics, techniques: image processing, galaxies: kinematics and dynamics, galaxies: photometry, galaxies: structure},
     year = 2002,
    month = jun,
   volume = 333,
    pages = {400-410},
      doi = {10.1046/j.1365-8711.2002.05412.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.333..400C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari08,
   author = {{Cappellari}, M.},
    title = "{Measuring the inclination and mass-to-light ratio of axisymmetric galaxies via anisotropic Jeans models of stellar kinematics}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.0042},
 keywords = {galaxies: elliptical and lenticular, cD , galaxies: evolution , galaxies: formation , galaxies: kinematics and dynamics , galaxies: structure},
     year = 2008,
    month = oct,
   volume = 390,
    pages = {71-86},
      doi = {10.1111/j.1365-2966.2008.13754.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390...71C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Richstone98,
   author = {{Richstone}, D.~O. and {Tremaine}, S.},
    title = "{Maximum-entropy models of galaxies}",
  journal = {\apj},
 keywords = {Distribution Functions, Elliptical Galaxies, Galactic Structure, Maximum Entropy Method, Statistical Mechanics, Stellar Luminosity, Astronomical Models, Computational Astrophysics, Galactic Evolution, Weighting Functions},
     year = 1988,
    month = apr,
   volume = 327,
    pages = {82-88},
      doi = {10.1086/166171},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...327...82R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Filippenko03,
   author = {{Filippenko}, A.~V. and {Ho}, L.~C.},
    title = "{A Low-Mass Central Black Hole in the Bulgeless Seyfert 1 Galaxy NGC 4395}",
  journal = {\apjl},
   eprint = {astro-ph/0303429},
 keywords = {Galaxies: Individual: NGC Number: NGC 4395, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Seyfert},
     year = 2003,
    month = may,
   volume = 588,
    pages = {L13-L16},
      doi = {10.1086/375361},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...588L..13F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Scott09,
   author = {{Scott}, N. and {Cappellari}, M. and {Davies}, R.~L. and {Bacon}, R. and 
	{de Zeeuw}, P.~T. and {Emsellem}, E. and {Falc{\'o}n-Barroso}, J. and 
	{Krajnovi{\'c}}, D. and {Kuntschner}, H. and {McDermid}, R.~M. and 
	{Peletier}, R.~F. and {Pipino}, A. and {Sarzi}, M. and {van den Bosch}, R.~C.~E. and 
	{van de Ven}, G. and {van Scherpenzeel}, E.},
    title = "{The SAURON Project - XIV. No escape from V$_{esc}$: a global and local parameter in early-type galaxy evolution}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0906.3321},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: abundances , galaxies: elliptical and lenticular, cD , galaxies: evolution , galaxies: formation},
     year = 2009,
    month = oct,
   volume = 398,
    pages = {1835-1857},
      doi = {10.1111/j.1365-2966.2009.15275.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.398.1835S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shapiro06,
   author = {{Shapiro}, K.~L. and {Cappellari}, M. and {de Zeeuw}, T. and 
	{McDermid}, R.~M. and {Gebhardt}, K. and {van den Bosch}, R.~C.~E. and 
	{Statler}, T.~S.},
    title = "{The black hole in NGC 3379: a comparison of gas and stellar dynamical mass measurements with HST and integral-field data}",
  journal = {\mnras},
   eprint = {astro-ph/0605479},
 keywords = {black hole physics: galaxies: elliptical and lenticular, cD: galaxies: individual: NGC 3379: galaxies: kinematics and dynamics: galaxies: nuclei, black hole physics, galaxies: elliptical and lenticular, cD, galaxies: individual: NGC 3379, galaxies: kinematics and dynamics, galaxies: nuclei},
     year = 2006,
    month = aug,
   volume = 370,
    pages = {559-579},
      doi = {10.1111/j.1365-2966.2006.10537.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370..559S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Krist95,
   author = {{Krist}, J.},
    title = "{Simulation of HST PSFs using Tiny Tim}",
booktitle = {Astronomical Data Analysis Software and Systems IV},
     year = 1995,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 77,
   editor = {{Shaw}, R.~A. and {Payne}, H.~E. and {Hayes}, J.~J.~E.},
    pages = {349},
   adsurl = {http://adsabs.harvard.edu/abs/1995ASPC...77..349K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vandermarel98,
   author = {{van der Marel}, R.~P. and {Cretton}, N. and {de Zeeuw}, P.~T. and 
	{Rix}, H.-W.},
    title = "{Improved Evidence for a Black Hole in M32 from HST/FOS Spectra. II. Axisymmetric Dynamical Models}",
  journal = {\apj},
   eprint = {astro-ph/9705081},
 keywords = {BLACK HOLE PHYSICS, GALAXIES: ELLIPTICAL AND LENTICULAR, CD, GALAXIES: INDIVIDUAL MESSIER NUMBER: M32, GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: NUCLEI, GALAXIES: STRUCTURE, Black Hole Physics, Galaxies: Elliptical and Lenticular, cD, Galaxies: Individual: Messier Number: M32, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Structure},
     year = 1998,
    month = jan,
   volume = 493,
    pages = {613-631},
      doi = {10.1086/305147},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...493..613V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Cappellari10,
   author = {{Cappellari}, M. and {McDermid}, R.~M. and {Bacon}, R. and {Davies}, R.~L. and 
	{de Zeeuw}, P.~T. and {Emsellem}, E. and {Falc{\'o}n-Barroso}, J. and 
	{Krajnovi{\'c}}, D. and {Kuntschner}, H. and {Peletier}, R.~F. and 
	{Sarzi}, M. and {van den Bosch}, R.~C.~E. and {van de Ven}, G.
	},
    title = "{Testing Mass Determinations of Supermassive Black Holes via Stellar Kinematics}",
 keywords = {black holes, mass measurement, merging, adaptive optics, Galactic nuclei circumnuclear matter and bulges, Masses and mass distribution, Galaxy mergers collisions and tidal interactions, Adaptive and segmented optics},
booktitle = {American Institute of Physics Conference Series},
     year = 2010,
   series = {American Institute of Physics Conference Series},
   volume = 1240,
archivePrefix = "arXiv",
   eprint = {1001.3233},
 primaryClass = "astro-ph.GA",
   editor = {{Debattista}, V.~P. and {Popescu}, C.~C.},
    month = jun,
    pages = {211-214},
      doi = {10.1063/1.3458489},
   adsurl = {http://adsabs.harvard.edu/abs/2010AIPC.1240..211C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Graham02,
   author = {{Graham}, A.~W.},
    title = "{Evidence for an Outer Disk in the Prototype ``Compact Elliptical'' Galaxy M32}",
  journal = {\apjl},
   eprint = {astro-ph/0202307},
 keywords = {Black Hole Physics, Galaxies: Bulges, Galaxies: Dwarf, Galaxies: Fundamental Parameters, Galaxies: Individual: Messier Number: M32, Galaxies: Structure},
     year = 2002,
    month = mar,
   volume = 568,
    pages = {L13-L17},
      doi = {10.1086/340274},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...568L..13G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kent87,
   author = {{Kent}, S.~M.},
    title = "{Surface photometry of six local group galaxies}",
  journal = {\aj},
 keywords = {Astronomical Photometry, Galactic Structure, Local Group (Astronomy), Andromeda Galaxy, Brightness Distribution, Galactic Nuclei, Mass To Light Ratios, Spectral Energy Distribution, Surface Properties},
     year = 1987,
    month = aug,
   volume = 94,
    pages = {306-314},
      doi = {10.1086/114472},
   adsurl = {http://adsabs.harvard.edu/abs/1987AJ.....94..306K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Graham08b,
   author = {{Graham}, A.~W.},
    title = "{Populating the Galaxy Velocity Dispersion - Supermassive Black Hole Mass Diagram: A Catalogue of (M$_{bh}$, {$\sigma$}) Values}",
  journal = {\pasa},
archivePrefix = "arXiv",
   eprint = {0807.2549},
 keywords = {catalogues, black hole physics, galaxies: bulges, galaxies: fundamental parameters, galaxies: kinematics and dynamics, galaxies: nuclei,},
     year = 2008,
    month = nov,
   volume = 25,
    pages = {167-175},
      doi = {10.1071/AS08013},
   adsurl = {http://adsabs.harvard.edu/abs/2008PASA...25..167G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Satyapal07,
   author = {{Satyapal}, S. and {Vega}, D. and {Heckman}, T. and {O'Halloran}, B. and 
	{Dudik}, R.},
    title = "{The Discovery of an Active Galactic Nucleus in the Late-Type Galaxy NGC 3621: Spitzer Spectroscopic Observations}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0706.1050},
 keywords = {Black Hole Physics, Galaxies: Active, Galaxies: Nuclei, Galaxies: Spiral, Infrared: Galaxies},
     year = 2007,
    month = jul,
   volume = 663,
    pages = {L9-L12},
      doi = {10.1086/519995},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...663L...9S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Green04,
   author = {{Greene}, J.~E. and {Ho}, L.~C.},
    title = "{Active Galactic Nuclei with Candidate Intermediate-Mass Black Holes}",
  journal = {\apj},
   eprint = {astro-ph/0404110},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert},
     year = 2004,
    month = aug,
   volume = 610,
    pages = {722-736},
      doi = {10.1086/421719},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...610..722G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Filippenko89,
   author = {{Filippenko}, A.~V. and {Sargent}, W.~L.~W.},
    title = "{Discovery of an extremely low luminosity Seyfert 1 nucleus in the dwarf galaxy NGC 4395}",
  journal = {\apjl},
 keywords = {Dwarf Galaxies, Galactic Nuclei, Light (Visible Radiation), Seyfert Galaxies, Stellar Luminosity, Emission Spectra, H Alpha Line, H Ii Regions, Line Spectra},
     year = 1989,
    month = jul,
   volume = 342,
    pages = {L11-L14},
      doi = {10.1086/185472},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...342L..11F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Volonteri08,
   author = {{Volonteri}, M. and {Lodato}, G. and {Natarajan}, P.},
    title = "{The evolution of massive black hole seeds}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0709.0529},
 keywords = {black hole physics , galaxies: evolution , quasars: general , cosmology: miscellaneous},
     year = 2008,
    month = jan,
   volume = 383,
    pages = {1079-1088},
      doi = {10.1111/j.1365-2966.2007.12589.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.383.1079V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kormendy95,
   author = {{Kormendy}, J. and {Richstone}, D.},
    title = "{Inward Bound---The Search For Supermassive Black Holes In Galactic Nuclei}",
  journal = {\araa},
     year = 1995,
   volume = 33,
    pages = {581},
      doi = {10.1146/annurev.aa.33.090195.003053},
   adsurl = {http://adsabs.harvard.edu/abs/1995ARA%26A..33..581K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Magorrian98,
   author = {{Magorrian}, J. and {Tremaine}, S. and {Richstone}, D. and {Bender}, R. and 
	{Bower}, G. and {Dressler}, A. and {Faber}, S.~M. and {Gebhardt}, K. and 
	{Green}, R. and {Grillmair}, C. and {Kormendy}, J. and {Lauer}, T.
	},
    title = "{The Demography of Massive Dark Objects in Galaxy Centers}",
  journal = {\aj},
   eprint = {astro-ph/9708072},
 keywords = {COSMOLOGY: DARK MATTER, GALAXIES: NUCLEI},
     year = 1998,
    month = jun,
   volume = 115,
    pages = {2285-2305},
      doi = {10.1086/300353},
   adsurl = {http://adsabs.harvard.edu/abs/1998AJ....115.2285M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Haring04,
   author = {{H{\"a}ring}, N. and {Rix}, H.-W.},
    title = "{On the Black Hole Mass-Bulge Mass Relation}",
  journal = {\apjl},
   eprint = {astro-ph/0402376},
 keywords = {Galaxies: Bulges, Galaxies: Kinematics and Dynamics},
     year = 2004,
    month = apr,
   volume = 604,
    pages = {L89-L92},
      doi = {10.1086/383567},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...604L..89H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ferrarese06,
   author = {{Ferrarese}, L. and {C{\^o}t{\'e}}, P. and {Dalla Bont{\`a}}, E. and 
	{Peng}, E.~W. and {Merritt}, D. and {Jord{\'a}n}, A. and {Blakeslee}, J.~P. and 
	{Ha{\c s}egan}, M. and {Mei}, S. and {Piatek}, S. and {Tonry}, J.~L. and 
	{West}, M.~J.},
    title = "{A Fundamental Relation between Compact Stellar Nuclei, Supermassive Black Holes, and Their Host Galaxies}",
  journal = {\apjl},
   eprint = {astro-ph/0603840},
 keywords = {Black Hole Physics, Galaxies: Elliptical and Lenticular, cD, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Structure},
     year = 2006,
    month = jun,
   volume = 644,
    pages = {L21-L24},
      doi = {10.1086/505388},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...644L..21F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ferrarese00a,
   author = {{Ferrarese}, L. and {Mould}, J.~R. and {Kennicutt}, Jr., R.~C. and 
	{Huchra}, J. and {Ford}, H.~C. and {Freedman}, W.~L. and {Stetson}, P.~B. and 
	{Madore}, B.~F. and {Sakai}, S. and {Gibson}, B.~K. and {Graham}, J.~A. and 
	{Hughes}, S.~M. and {Illingworth}, G.~D. and {Kelson}, D.~D. and 
	{Macri}, L. and {Sebo}, K. and {Silbermann}, N.~A.},
    title = "{The Hubble Space Telescope Key Project on the Extragalactic Distance Scale. XXVI. The Calibration of Population II Secondary Distance Indicators and the Value of the Hubble Constant}",
  journal = {\apj},
   eprint = {astro-ph/9908192},
 keywords = {SUBJECT HEADINGS: STARS: VARIABLES: CEPHEIDS, COSMOLOGY: DISTANCE SCALE, GALAXIES: STAR CLUSTERS, STARS: LATE-TYPE, Subject headings: Stars: Variables: Cepheids, Cosmology: Distance Scale, Galaxies: Star Clusters, Stars: Late-Type},
     year = 2000,
    month = feb,
   volume = 529,
    pages = {745-767},
      doi = {10.1086/308309},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...529..745F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ferrarese00b,
   author = {{Ferrarese}, L. and {Merritt}, D.},
    title = "{A Fundamental Relation between Supermassive Black Holes and Their Host Galaxies}",
  journal = {\apjl},
   eprint = {astro-ph/0006053},
 keywords = {Black Hole Physics, Galaxies: Evolution, Galaxies: Kinematics and Dynamics},
     year = 2000,
    month = aug,
   volume = 539,
    pages = {L9-L12},
      doi = {10.1086/312838},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...539L...9F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gebhardt00,
   author = {{Gebhardt}, K. and {Bender}, R. and {Bower}, G. and {Dressler}, A. and 
	{Faber}, S.~M. and {Filippenko}, A.~V. and {Green}, R. and {Grillmair}, C. and 
	{Ho}, L.~C. and {Kormendy}, J. and {Lauer}, T.~R. and {Magorrian}, J. and 
	{Pinkney}, J. and {Richstone}, D. and {Tremaine}, S.},
    title = "{A Relationship between Nuclear Black Hole Mass and Galaxy Velocity Dispersion}",
  journal = {\apjl},
   eprint = {astro-ph/0006289},
 keywords = {Galaxies: General, Galaxies: Nuclei, Galaxies: Statistics},
     year = 2000,
    month = aug,
   volume = 539,
    pages = {L13-L16},
      doi = {10.1086/312840},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...539L..13G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wehner06,
   author = {{Wehner}, E.~H. and {Harris}, W.~E.},
    title = "{From Supermassive Black Holes to Dwarf Elliptical Nuclei: A Mass Continuum}",
  journal = {\apjl},
   eprint = {astro-ph/0603801},
 keywords = {Black Hole Physics, Galaxies: Bulges, Galaxies: Dwarf, Galaxies: Fundamental Parameters, Galaxies: Nuclei-},
     year = 2006,
    month = jun,
   volume = 644,
    pages = {L17-L20},
      doi = {10.1086/505387},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...644L..17W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rossa06,
   author = {{Rossa}, J. and {van der Marel}, R.~P. and {B{\"o}ker}, T. and 
	{Gerssen}, J. and {Ho}, L.~C. and {Rix}, H.-W. and {Shields}, J.~C. and 
	{Walcher}, C.-J.},
    title = "{Hubble Space Telescope STIS Spectra of Nuclear Star Clusters in Spiral Galaxies: Dependence of Age and Mass on Hubble Type}",
  journal = {\aj},
   eprint = {astro-ph/0604140},
 keywords = {Galaxies: Evolution, Galaxies: Nuclei, Galaxies: Spiral, Galaxies: Star Clusters, Galaxies: Stellar Content},
     year = 2006,
    month = sep,
   volume = 132,
    pages = {1074-1099},
      doi = {10.1086/505968},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....132.1074R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cote06,
   author = {{C{\^o}t{\'e}}, P. and {Piatek}, S. and {Ferrarese}, L. and 
	{Jord{\'a}n}, A. and {Merritt}, D. and {Peng}, E.~W. and {Ha{\c s}egan}, M. and 
	{Blakeslee}, J.~P. and {Mei}, S. and {West}, M.~J. and {Milosavljevi{\'c}}, M. and 
	{Tonry}, J.~L.},
    title = "{The ACS Virgo Cluster Survey. VIII. The Nuclei of Early-Type Galaxies}",
  journal = {\apjs},
   eprint = {astro-ph/0603252},
 keywords = {Galaxies: Clusters: Individual: Name: Virgo, Galaxies: Elliptical and Lenticular, cD, Galaxies: Nuclei, Galaxies: Structure},
     year = 2006,
    month = jul,
   volume = 165,
    pages = {57-94},
      doi = {10.1086/504042},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..165...57C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Graham09,
   author = {{Graham}, A.~W. and {Spitler}, L.~R.},
    title = "{Quantifying the coexistence of massive black holes and dense nuclear star clusters}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0907.5250},
 primaryClass = "astro-ph.CO",
 keywords = {black hole physics , galaxies: nuclei , galaxies: structure},
     year = 2009,
    month = aug,
   volume = 397,
    pages = {2148-2162},
      doi = {10.1111/j.1365-2966.2009.15118.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397.2148G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Long02,
   author = {{Long}, K.~S. and {Charles}, P.~A. and {Dubus}, G.},
    title = "{Hubble Space Telescope Spectroscopy of the Nucleus of M33}",
  journal = {\apj},
 keywords = {Galaxies: Individual: Messier Number: M33, Galaxies: Nuclei, Galaxies: Stellar Content, Galaxies: Local Group, Ultraviolet: Stars},
     year = 2002,
    month = apr,
   volume = 569,
    pages = {204-213},
      doi = {10.1086/339172},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...569..204L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boker02,
   author = {{B{\"o}ker}, T. and {Laine}, S. and {van der Marel}, R.~P. and 
	{Sarzi}, M. and {Rix}, H.-W. and {Ho}, L.~C. and {Shields}, J.~C.
	},
    title = "{A Hubble Space Telescope Census of Nuclear Star Clusters in Late-Type Spiral Galaxies. I. Observations and Image Analysis}",
  journal = {\aj},
   eprint = {astro-ph/0112086},
 keywords = {Galaxies: Nuclei, Galaxies: Spiral, Galaxies: Star Clusters, Galaxies: Statistics, Galaxies: Structure},
     year = 2002,
    month = mar,
   volume = 123,
    pages = {1389-1410},
      doi = {10.1086/339025},
   adsurl = {http://adsabs.harvard.edu/abs/2002AJ....123.1389B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carollo02,
   author = {{Carollo}, C.~M. and {Stiavelli}, M. and {Seigar}, M. and {de Zeeuw}, P.~T. and 
	{Dejonghe}, H.},
    title = "{Spiral Galaxies with HST/NICMOS. I. Nuclear Morphologies, Color Maps, and Distinct Nuclei}",
  journal = {\aj},
   eprint = {astro-ph/0110281},
 keywords = {Galaxies: Bulges, Galaxies: Evolution, Galaxies: Formation, Galaxies: Nuclei, Galaxies: Spiral, Galaxies: Structure},
     year = 2002,
    month = jan,
   volume = 123,
    pages = {159-183},
      doi = {10.1086/324725},
   adsurl = {http://adsabs.harvard.edu/abs/2002AJ....123..159C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shields08,
   author = {{Shields}, J.~C. and {Walcher}, C.~J. and {B{\"o}ker}, T. and 
	{Ho}, L.~C. and {Rix}, H.-W. and {van der Marel}, R.~P.},
    title = "{An Accreting Black Hole in the Nuclear Star Cluster of the Bulgeless Galaxy NGC 1042}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0804.4024},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Star Clusters},
     year = 2008,
    month = jul,
   volume = 682,
    pages = {104-109},
      doi = {10.1086/589680},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...682..104S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hopkins10a,
   author = {{Hopkins}, P.~F. and {Quataert}, E.},
    title = "{The nuclear stellar disc in Andromeda: a fossil from the era of black hole growth}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1002.1079},
 keywords = {galaxies: active, quasars: general, galaxies: evolution, cosmology: theory},
     year = 2010,
    month = jun,
   volume = 405,
    pages = {L41-L45},
      doi = {10.1111/j.1745-3933.2010.00855.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.405L..41H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ghez08,
   author = {{Ghez}, A.~M. and {Salim}, S. and {Weinberg}, N.~N. and {Lu}, J.~R. and 
	{Do}, T. and {Dunn}, J.~K. and {Matthews}, K. and {Morris}, M.~R. and 
	{Yelda}, S. and {Becklin}, E.~E. and {Kremenek}, T. and {Milosavljevic}, M. and 
	{Naiman}, J.},
    title = "{Measuring Distance and Properties of the Milky Way's Central Supermassive Black Hole with Stellar Orbits}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0808.2870},
 keywords = {Black Hole Physics, Galaxy: Center, Galaxy: Kinematics and Dynamics, Infrared: Stars, Techniques: High Angular Resolution},
     year = 2008,
    month = dec,
   volume = 689,
    pages = {1044-1062},
      doi = {10.1086/592738},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...689.1044G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lu09,
   author = {{Lu}, J.~R. and {Ghez}, A.~M. and {Hornstein}, S.~D. and {Morris}, M.~R. and 
	{Becklin}, E.~E. and {Matthews}, K.},
    title = "{A Disk of Young Stars at the Galactic Center as Determined by Individual Stellar Orbits}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0808.3818},
 keywords = {black hole physics, Galaxy: center, infrared: stars, techniques: high angular resolution},
     year = 2009,
    month = jan,
   volume = 690,
    pages = {1463-1487},
      doi = {10.1088/0004-637X/690/2/1463},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690.1463L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bartko09,
   author = {{Bartko}, H. and {Martins}, F. and {Fritz}, T.~K. and {Genzel}, R. and 
	{Levin}, Y. and {Perets}, H.~B. and {Paumard}, T. and {Nayakshin}, S. and 
	{Gerhard}, O. and {Alexander}, T. and {Dodds-Eden}, K. and {Eisenhauer}, F. and 
	{Gillessen}, S. and {Mascetti}, L. and {Ott}, T. and {Perrin}, G. and 
	{Pfuhl}, O. and {Reid}, M.~J. and {Rouan}, D. and {Sternberg}, A. and 
	{Trippe}, S.},
    title = "{Evidence for Warped Disks of Young Stars in the Galactic Center}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0811.3903},
 keywords = {Galaxy: center, stars: early-type, stars: formation, stars: luminosity function, mass function, stellar dynamics},
     year = 2009,
    month = jun,
   volume = 697,
    pages = {1741-1763},
      doi = {10.1088/0004-637X/697/2/1741},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...697.1741B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tikhonov03,
   author = {{Tikhonov}, N.~A. and {Galazutdinova}, O.~A. and {Aparicio}, A.
	},
    title = "{Stellar content of NGC 404 - The nearest S0 Galaxy}",
  journal = {\aap},
 keywords = {galaxies: individual: NGC 404, galaxies: stellar content, galaxies: photometry, galaxies: distance and redshifts},
     year = 2003,
    month = apr,
   volume = 401,
    pages = {863-872},
      doi = {10.1051/0004-6361:20021819},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...401..863T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wiklind90,
   author = {{Wiklind}, T. and {Henkel}, C.},
    title = "{The molecular cloud content of early type galaxies. II - A molecular ring in NGC 404}",
  journal = {\aap},
 keywords = {Elliptical Galaxies, Galactic Evolution, Molecular Clouds, Astronomical Spectroscopy, Carbon Monoxide, Cosmic Dust, Galactic Structure, Star Formation, Thermal Emission},
     year = 1990,
    month = jan,
   volume = 227,
    pages = {394-406},
   adsurl = {http://adsabs.harvard.edu/abs/1990A%26A...227..394W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ravindranath01,
   author = {{Ravindranath}, S. and {Ho}, L.~C. and {Peng}, C.~Y. and {Filippenko}, A.~V. and 
	{Sargent}, W.~L.~W.},
    title = "{Central Structural Parameters of Early-Type Galaxies as Viewed with Nicmos on the Hubble Space Telescope}",
  journal = {\aj},
   eprint = {astro-ph/0105390},
 keywords = {Galaxies: Active, Galaxies: Elliptical and Lenticular, cD, Galaxies: Nuclei, Galaxies: Photometry, Galaxies: Seyfert, Galaxy: Structure},
     year = 2001,
    month = aug,
   volume = 122,
    pages = {653-678},
      doi = {10.1086/321175},
   adsurl = {http://adsabs.harvard.edu/abs/2001AJ....122..653R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Genzel96,
   author = {{Genzel}, R. and {Thatte}, N. and {Krabbe}, A. and {Kroker}, H. and 
	{Tacconi-Garman}, L.~E.},
    title = "{The Dark Mass Concentration in the Central Parsec of the Milky Way}",
  journal = {\apj},
 keywords = {CELESTIAL MECHANICS, STELLAR DYNAMICS, GALAXY: CENTER, INFRARED: STARS, TECHNIQUES: RADIAL VELOCITIES},
     year = 1996,
    month = nov,
   volume = 472,
    pages = {153},
      doi = {10.1086/178051},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...472..153G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schodel07,
   author = {{Sch{\"o}del}, R. and {Eckart}, A. and {Alexander}, T. and {Merritt}, D. and 
	{Genzel}, R. and {Sternberg}, A. and {Meyer}, L. and {Kul}, F. and 
	{Moultaka}, J. and {Ott}, T. and {Straubmeier}, C.},
    title = "{The structure of the nuclear stellar cluster of the Milky Way}",
  journal = {\aap},
   eprint = {astro-ph/0703178},
 keywords = {stellar dynamics, Galaxy: centre, Galaxy: nucleus, infrared: stars},
     year = 2007,
    month = jul,
   volume = 469,
    pages = {125-146},
      doi = {10.1051/0004-6361:20065089},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..125S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Trippe08,
   author = {{Trippe}, S. and {Gillessen}, S. and {Gerhard}, O.~E. and {Bartko}, H. and 
	{Fritz}, T.~K. and {Maness}, H.~L. and {Eisenhauer}, F. and 
	{Martins}, F. and {Ott}, T. and {Dodds-Eden}, K. and {Genzel}, R.
	},
    title = "{Kinematics of the old stellar population at the Galactic centre}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0810.1040},
 keywords = {Galaxy: center, Galaxy: kinematics and dynamics, stars: kinematics, infrared: stars},
     year = 2008,
    month = dec,
   volume = 492,
    pages = {419-439},
      doi = {10.1051/0004-6361:200810191},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...492..419T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Greene04,
   author = {{Greene}, J.~E. and {Ho}, L.~C.},
    title = "{Active Galactic Nuclei with Candidate Intermediate-Mass Black Holes}",
  journal = {\apj},
   eprint = {astro-ph/0404110},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert},
     year = 2004,
    month = aug,
   volume = 610,
    pages = {722-736},
      doi = {10.1086/421719},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...610..722G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Richstone88,
   author = {{Richstone}, D.~O. and {Tremaine}, S.},
    title = "{Maximum-entropy models of galaxies}",
  journal = {\apj},
 keywords = {Distribution Functions, Elliptical Galaxies, Galactic Structure, Maximum Entropy Method, Statistical Mechanics, Stellar Luminosity, Astronomical Models, Computational Astrophysics, Galactic Evolution, Weighting Functions},
     year = 1988,
    month = apr,
   volume = 327,
    pages = {82-88},
      doi = {10.1086/166171},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...327...82R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McKernan11,
   author = {{McKernan}, B. and {Ford}, K.~E.~S. and {Yaqoob}, T. and {Winter}, L.~M.
	},
    title = "{On minor black holes in galactic nuclei}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1102.0260},
 primaryClass = "astro-ph.CO",
 keywords = {accretion, accretion discs, techniques: high angular resolution, stars: formation, galaxies: active, galaxies: nuclei, X-rays: galaxies},
     year = 2011,
    month = may,
   volume = 413,
    pages = {L24-L28},
      doi = {10.1111/j.1745-3933.2011.01024.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.413L..24M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004cbhg.symp...37V,
   author = {{van der Marel}, R.~P.},
    title = "{Intermediate-mass Black Holes in the Universe: A Review of Formation Theories and Observational Constraints}",
  journal = {Coevolution of Black Holes and Galaxies},
   eprint = {astro-ph/0302101},
     year = 2004,
    pages = {37},
   adsurl = {http://adsabs.harvard.edu/abs/2004cbhg.symp...37V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Volonteri10,
   author = {{Volonteri}, M.},
    title = "{Formation of supermassive black holes}",
  journal = {\aapr},
archivePrefix = "arXiv",
   eprint = {1003.4404},
 primaryClass = "astro-ph.CO",
 keywords = {Black hole physics, Galaxies: formation, Cosmology: theory, Quasars, Galaxies: evolution},
     year = 2010,
    month = jul,
   volume = 18,
    pages = {279-315},
      doi = {10.1007/s00159-010-0029-x},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26ARv..18..279V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanWassenhove10,
   author = {{van Wassenhove}, S. and {Volonteri}, M. and {Walker}, M.~G. and 
	{Gair}, J.~R.},
    title = "{Massive black holes lurking in Milky Way satellites}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1001.5451},
 primaryClass = "astro-ph.CO",
 keywords = {black hole physics, galaxies: dwarf, galaxies: evolution, galaxies: formation, cosmology: theory},
     year = 2010,
    month = oct,
   volume = 408,
    pages = {1139-1146},
      doi = {10.1111/j.1365-2966.2010.17189.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.408.1139V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hughes09,
   author = {{Hughes}, S.~A.},
    title = "{Gravitational Waves from Merging Compact Binaries}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0903.4877},
 primaryClass = "astro-ph.CO",
     year = 2009,
    month = sep,
   volume = 47,
    pages = {107-157},
      doi = {10.1146/annurev-astro-082708-101711},
   adsurl = {http://adsabs.harvard.edu/abs/2009ARA%26A..47..107H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nguyen14,
   author = {{Nguyen}, D.~D. and {Seth}, A.~C. and {Reines}, A.~E. and {den Brok}, M. and 
	{Sand}, D. and {McLeod}, B.},
    title = "{Extended Structure and Fate of the Nucleus in Henize 2-10}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1408.4446},
 keywords = {methods: data analysis, surveys, techniques: spectroscopic},
     year = 2014,
    month = oct,
   volume = 794,
      eid = {34},
    pages = {34},
      doi = {10.1088/0004-637X/794/1/34},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...794...34N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vandermarel04review,
   author = {{van der Marel}, R.~P.},
    title = "{Intermediate-mass Black Holes in the Universe: A Review of Formation Theories and Observational Constraints}",
  journal = {Coevolution of Black Holes and Galaxies},
   eprint = {astro-ph/0302101},
     year = 2004,
    pages = {37},
   adsurl = {http://adsabs.harvard.edu/abs/2004cbhg.symp...37V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Peterson05,
   author = {{Peterson}, B.~M. and {Bentz}, M.~C. and {Desroches}, L.-B. and 
	{Filippenko}, A.~V. and {Ho}, L.~C. and {Kaspi}, S. and {Laor}, A. and 
	{Maoz}, D. and {Moran}, E.~C. and {Pogge}, R.~W. and {Quillen}, A.~C.
	},
    title = "{Multiwavelength Monitoring of the Dwarf Seyfert 1 Galaxy NGC 4395. I. A Reverberation-based Measurement of the Black Hole Mass}",
  journal = {\apj},
   eprint = {astro-ph/0506665},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Quasars: Emission Lines, Ultraviolet: Galaxies},
     year = 2005,
    month = oct,
   volume = 632,
    pages = {799-808},
      doi = {10.1086/444494},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...632..799P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barth04,
   author = {{Barth}, A.~J. and {Ho}, L.~C. and {Rutledge}, R.~E. and {Sargent}, W.~L.~W.
	},
    title = "{POX 52: A Dwarf Seyfert 1 Galaxy with an Intermediate-Mass Black Hole}",
  journal = {\apj},
   eprint = {astro-ph/0402110},
 keywords = {Galaxies: Active, Galaxies: Dwarf, Galaxies: Individual: Alphanumeric: POX 52, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Seyfert},
     year = 2004,
    month = may,
   volume = 607,
    pages = {90-102},
      doi = {10.1086/383302},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...607...90B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barth02b,
   author = {{Barth}, A.~J. and {Ho}, L.~C. and {Sargent}, W.~L.~W.},
    title = "{A Study of the Direct Fitting Method for Measurement of Galaxy Velocity Dispersions}",
  journal = {\aj},
   eprint = {astro-ph/0209564},
 keywords = {Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Techniques: Spectroscopic},
     year = 2002,
    month = nov,
   volume = 124,
    pages = {2607-2614},
      doi = {10.1086/343840},
   adsurl = {http://adsabs.harvard.edu/abs/2002AJ....124.2607B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barth02a,
   author = {{Barth}, A.~J. and {Ho}, L.~C. and {Sargent}, W.~L.~W.},
    title = "{Stellar Velocity Dispersion and Black Hole Mass in the Blazar Markarian 501}",
  journal = {\apjl},
   eprint = {astro-ph/0201064},
 keywords = {Galaxies: BL Lacertae Objects: Individual: Name: Markarian 501, Galaxies: Active, Galaxies: Elliptical and Lenticular, cD, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei},
     year = 2002,
    month = feb,
   volume = 566,
    pages = {L13-L16},
      doi = {10.1086/339452},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...566L..13B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Thornton08,
   author = {{Thornton}, C.~E. and {Barth}, A.~J. and {Ho}, L.~C. and {Rutledge}, R.~E. and 
	{Greene}, J.~E.},
    title = "{The Host Galaxy and Central Engine of the Dwarf Active Galactic Nucleus POX 52}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0807.1535},
 keywords = {Galaxies: Active, Galaxies: Dwarf, Galaxies: Individual: Alphanumeric: POX 52, Galaxies: Nuclei, Galaxies: Seyfert, X-Rays: Galaxies},
     year = 2008,
    month = oct,
   volume = 686,
    pages = {892-910},
      doi = {10.1086/591519},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...686..892T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McAlpine11,
   author = {{McAlpine}, W. and {Satyapal}, S. and {Gliozzi}, M. and {Cheung}, C.~C. and 
	{Sambruna}, R.~M. and {Eracleous}, M.},
    title = "{Black Holes in Bulgeless Galaxies: An XMM-Newton Investigation of NGC 3367 and NGC 4536}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1012.0834},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: active, galaxies: starburst, infrared: galaxies, X-rays: galaxies},
     year = 2011,
    month = feb,
   volume = 728,
      eid = {25},
    pages = {25},
      doi = {10.1088/0004-637X/728/1/25},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...728...25M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ho04review,
   author = {{Ho}, L.~C.~W.},
    title = "{Black Hole Demography from Nearby Active Galactic Nuclei}",
  journal = {Coevolution of Black Holes and Galaxies},
   eprint = {astro-ph/0401527},
     year = 2004,
    pages = {292},
   adsurl = {http://adsabs.harvard.edu/abs/2004cbhg.symp..292H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Kormendy93review,
   author = {{Kormendy}, J.},
    title = "{A critical review of stellar-dynamical evidence for black holes in galaxy nuclei}",
booktitle = {The Nearest Active Galaxies},
     year = 1993,
   editor = {{Beckman}, J. and {Colina}, L. and {Netzer}, H.},
    month = jan,
    pages = {197-218},
   adsurl = {http://adsabs.harvard.edu/abs/1993nag..conf..197K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Kormendy01,
   author = {{Kormendy}, J. and {Gebhardt}, K.},
    title = "{Supermassive black holes in galactic nuclei}",
 keywords = {Galactic nuclei circumnuclear matter and bulges, Spiral galaxies, Black holes},
booktitle = {20th Texas Symposium on relativistic astrophysics},
     year = 2001,
   series = {American Institute of Physics Conference Series},
   volume = 586,
   eprint = {astro-ph/0105230},
   editor = {{Wheeler}, J.~C. and {Martel}, H.},
    month = oct,
    pages = {363-381},
      doi = {10.1063/1.1419581},
   adsurl = {http://adsabs.harvard.edu/abs/2001AIPC..586..363K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baldry04,
   author = {{Baldry}, I.~K. and {Glazebrook}, K. and {Brinkmann}, J. and 
	{Ivezi{\'c}}, {\v Z}. and {Lupton}, R.~H. and {Nichol}, R.~C. and 
	{Szalay}, A.~S.},
    title = "{Quantifying the Bimodal Color-Magnitude Distribution of Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/0309710},
 keywords = {Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: Luminosity Function, Mass Function, Galaxies: Photometry},
     year = 2004,
    month = jan,
   volume = 600,
    pages = {681-694},
      doi = {10.1086/380092},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...600..681B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Thilker10,
   author = {{Thilker}, D.~A. and {Bianchi}, L. and {Schiminovich}, D. and 
	{Gil de Paz}, A. and {Seibert}, M. and {Madore}, B.~F. and {Wyder}, T. and 
	{Rich}, R.~M. and {Yi}, S. and {Barlow}, T. and {Conrow}, T. and 
	{Forster}, K. and {Friedman}, P. and {Martin}, C. and {Morrissey}, P. and 
	{Neff}, S. and {Small}, T.},
    title = "{NGC 404: A Rejuvenated Lenticular Galaxy on a Merger-induced, Blueward Excursion Into the Green Valley}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1003.4985},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: individual: NGC 404, galaxies: interactions, galaxies: structure},
     year = 2010,
    month = may,
   volume = 714,
    pages = {L171-L175},
      doi = {10.1088/2041-8205/714/1/L171},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714L.171T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schlafly11,
   author = {{Schlafly}, E.~F. and {Finkbeiner}, D.~P.},
    title = "{Measuring Reddening with Sloan Digital Sky Survey Stellar Spectra and Recalibrating SFD}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1012.4804},
 primaryClass = "astro-ph.GA",
 keywords = {dust, extinction, Galaxy: stellar content, ISM: clouds},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {103},
    pages = {103},
      doi = {10.1088/0004-637X/737/2/103},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737..103S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Denbrok13abstract,
   author = {{Den Brok}, M. and {Seth}, A. and {Barth}, A. and {Neumayer}, N.
	},
    title = "{A Dynamical Mass Estimate of the Intermediate Mass Black Hole in NGC4395}",
booktitle = {SnowPAC 2013 - Black Hole Fingerprints: Dynamics, Disruptions and Demographics},
     year = 2013,
    month = mar,
      eid = {59},
    pages = {59},
   adsurl = {http://adsabs.harvard.edu/abs/2013snpa.confE..59D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kormendy13,
   author = {{Kormendy}, J. and {Ho}, L.~C.},
    title = "{Coevolution (Or Not) of Supermassive Black Holes and Host Galaxies}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1304.7762},
 primaryClass = "astro-ph.CO",
     year = 2013,
    month = aug,
   volume = 51,
    pages = {511-653},
      doi = {10.1146/annurev-astro-082708-101811},
   adsurl = {http://adsabs.harvard.edu/abs/2013ARA%26A..51..511K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kormendy09,
   author = {{Kormendy}, J. and {Bender}, R.},
    title = "{Correlations between Supermassive Black Holes, Velocity Dispersions, and Mass Deficits in Elliptical Galaxies with Cores}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0901.3778},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: nuclei, galaxies: photometry, galaxies: structure},
     year = 2009,
    month = feb,
   volume = 691,
    pages = {L142-L146},
      doi = {10.1088/0004-637X/691/2/L142},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...691L.142K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kriek10,
   author = {{Kriek}, M. and {Labb{\'e}}, I. and {Conroy}, C. and {Whitaker}, K.~E. and 
	{van Dokkum}, P.~G. and {Brammer}, G.~B. and {Franx}, M. and 
	{Illingworth}, G.~D. and {Marchesini}, D. and {Muzzin}, A. and 
	{Quadri}, R.~F. and {Rudnick}, G.},
    title = "{The Spectral Energy Distribution of Post-starburst Galaxies in the NEWFIRM Medium-band Survey: A Low Contribution from TP-AGB Stars}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1008.4357},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: stellar content, stars: AGB and post-AGB},
     year = 2010,
    month = oct,
   volume = 722,
    pages = {L64-L69},
      doi = {10.1088/2041-8205/722/1/L64},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...722L..64K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@TECHREPORT{Brown08,
   author = {{Brown}, T.~M. and {Hartig}, G. and {Baggett}, S.},
    title = "{WFC3 TV3 Testing: UVIS Window Contamination}",
 keywords = {Hubble Space Telescope, HST, Space Telescope Science Institute, Wide Field Camera 3, WFC3, thermal vacuum testing, UVIS flight detector},
booktitle = {Space Telescope WFC Instrument Science Report},
     year = 2008,
    month = may,
    pages = {10},
   adsurl = {http://adsabs.harvard.edu/abs/2008wfc..rept...10B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@TECHREPORT{Hartig08,
   author = {{Hartig}, G.~F.},
    title = "{WFC3 UVIS PSF Evaluation in Thermal-Vacuum Test \#3}",
 keywords = {Hubble Space Telescope, HST, Space Telescope Science Institute, WFC3, Wide Field Camera 3, UVIS PSF Evaluation},
booktitle = {Space Telescope WFC Instrument Science Report},
     year = 2008,
    month = aug,
    pages = {40},
   adsurl = {http://adsabs.harvard.edu/abs/2008wfc..rept...40H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Seth14,
   author = {{Seth}, A.~C. and {van den Bosch}, R. and {Mieske}, S. and {Baumgardt}, H. and 
	{Brok}, M.~D. and {Strader}, J. and {Neumayer}, N. and {Chilingarian}, I. and 
	{Hilker}, M. and {McDermid}, R. and {Spitler}, L. and {Brodie}, J. and 
	{Frank}, M.~J. and {Walsh}, J.~L.},
    title = "{A supermassive black hole in an ultra-compact dwarf galaxy}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1409.4769},
     year = 2014,
    month = sep,
   volume = 513,
    pages = {398-400},
      doi = {10.1038/nature13762},
   adsurl = {http://adsabs.harvard.edu/abs/2014Natur.513..398S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Greene07,
   author = {{Greene}, J.~E. and {Ho}, L.~C.},
    title = "{A New SAMPLE of Low-Mass Black Holes in ACTIVE Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0707.2617},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert},
     year = 2007,
    month = nov,
   volume = 670,
    pages = {92-104},
      doi = {10.1086/522082},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...670...92G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}  
  
@ARTICLE{Noyola08,
   author = {{Noyola}, E. and {Gebhardt}, K. and {Bergmann}, M.},
    title = "{Gemini and Hubble Space Telescope Evidence for an Intermediate-Mass Black Hole in {$\omega$} Centauri}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0801.2782},
 keywords = {Black Hole Physics, Galaxy: Globular Clusters: Individual: Name: {$\omega$} Centauri, Stellar Dynamics},
     year = 2008,
    month = apr,
   volume = 676,
    pages = {1008-1015},
      doi = {10.1086/529002},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...676.1008N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ibata09,
   author = {{Ibata}, R. and {Bellazzini}, M. and {Chapman}, S.~C. and {Dalessandro}, E. and 
	{Ferraro}, F. and {Irwin}, M. and {Lanzoni}, B. and {Lewis}, G.~F. and 
	{Mackey}, A.~D. and {Miocchi}, P. and {Varghese}, A.},
    title = "{Density and Kinematic Cusps in M54 at the Heart of the Sagittarius Dwarf Galaxy: Evidence for A 10$^{4}$ M $_{sun}$ Black Hole?}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0906.4894},
 primaryClass = "astro-ph.GA",
 keywords = {black hole physics, globular clusters: individual: M54, stellar dynamics},
     year = 2009,
    month = jul,
   volume = 699,
    pages = {L169-L173},
      doi = {10.1088/0004-637X/699/2/L169},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...699L.169I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanderMarel10,
   author = {{van der Marel}, R.~P. and {Anderson}, J.},
    title = "{New Limits on an Intermediate-Mass Black Hole in Omega Centauri. II. Dynamical Models}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0905.0638},
 primaryClass = "astro-ph.GA",
 keywords = {globular clusters: individual: omega Centauri, stars: kinematics and dynamics},
     year = 2010,
    month = feb,
   volume = 710,
    pages = {1063-1088},
      doi = {10.1088/0004-637X/710/2/1063},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710.1063V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Antonini13,
   author = {{Antonini}, F.},
    title = "{Origin and Growth of Nuclear Star Clusters around Massive Black Holes}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1207.6589},
 keywords = {galaxies: nuclei, Galaxy: center, Galaxy: formation, Galaxy: kinematics and dynamics, Galaxy: nucleus, globular clusters: general},
     year = 2013,
    month = jan,
   volume = 763,
      eid = {62},
    pages = {62},
      doi = {10.1088/0004-637X/763/1/62},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...763...62A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{denBrok14,
   author = {{den Brok}, M. and {Peletier}, R.~F. and {Seth}, A. and {Balcells}, M. and 
	{Dominguez}, L. and {Graham}, A.~W. and {Carter}, D. and {Erwin}, P. and 
	{Ferguson}, H.~C. and {Goudfrooij}, P. and {Guzm{\'a}n}, R. and 
	{Hoyos}, C. and {Jogee}, S. and {Lucey}, J. and {Phillipps}, S. and 
	{Puzia}, T. and {Valentijn}, E. and {Kleijn}, G.~V. and {Weinzirl}, T.
	},
    title = "{The HST/ACS Coma Cluster SURVEY - X. Nuclear star clusters in low-mass early-type galaxies: scaling relations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1409.4766},
 keywords = {galaxies: dwarf, galaxies: nuclei, galaxies: star clusters: general},
     year = 2014,
    month = dec,
   volume = 445,
    pages = {2385-2403},
      doi = {10.1093/mnras/stu1906},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.445.2385D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hopkins09,
   author = {{Hopkins}, P.~F. and {Murray}, N. and {Thompson}, T.~A.},
    title = "{The small scatter in BH-host correlations and the case for self-regulated BH growth}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0903.3949},
 keywords = {galaxies: ACTIVE , galaxies: evolution , galaxies: formation , quasars: general , cosmology: theory},
     year = 2009,
    month = sep,
   volume = 398,
    pages = {303-311},
      doi = {10.1111/j.1365-2966.2009.15132.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.398..303H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Williams.M.J10,
   author = {{Williams}, M.~J. and {Bureau}, M. and {Cappellari}, M.},
    title = "{The Tully-Fisher relations of early-type spiral and S0 galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1007.4072},
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: kinematics and dynamics, galaxies: spiral, galaxies: structure},
     year = 2010,
    month = dec,
   volume = 409,
    pages = {1330-1346},
      doi = {10.1111/j.1365-2966.2010.17406.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.409.1330W},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Williams.B.F10,
   author = {{Williams}, B.~F. and {Dalcanton}, J.~J. and {Gilbert}, K.~M. and 
	{Stilp}, A. and {Dolphin}, A. and {Seth}, A.~C. and {Weisz}, D. and 
	{Skillman}, E.},
    title = "{The Advanced Camera for SURVEYS Nearby Galaxy Survey Treasury. VI. The Ancient Star-forming Disk of NGC 404}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1004.5135},
 keywords = {galaxies: evolution, galaxies: individual: NGC 404, galaxies: stellar content},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {71-83},
      doi = {10.1088/0004-637X/716/1/71},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716...71W},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Reines13,
   author = {{Reines}, A.~E. and {Greene}, J.~E. and {Geha}, M.},
    title = "{Dwarf Galaxies with Optical Signatures of ACTIVE Massive Black Holes}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1308.0328},
 keywords = {galaxies: ACTIVE, galaxies: dwarf, galaxies: nuclei, galaxies: Seyfert},
     year = 2013,
    month = oct,
   volume = 775,
      eid = {116},
    pages = {116},
      doi = {10.1088/0004-637X/775/2/116},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...775..116R},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Moran14,
   author = {{Moran}, E.~C. and {Shahinyan}, K. and {Sugarman}, H.~R. and 
	{V{\'e}lez}, D.~O. and {Eracleous}, M.},
    title = "{Black Holes At the Centers of Nearby Dwarf Galaxies}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1408.4451},
 keywords = {galaxies: ACTIVE, galaxies: dwarf, galaxies: Seyfert},
     year = 2014,
    month = dec,
   volume = 148,
      eid = {136},
    pages = {136},
      doi = {10.1088/0004-6256/148/6/136},
   adsurl = {http://adsabs.harvard.edu/abs/2014AJ....148..136M},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Gezari12,
   author = {{Gezari}, S. and {Chornock}, R. and {Rest}, A. and {Huber}, M.~E. and 
	{Forster}, K. and {Berger}, E. and {Challis}, P.~J. and {Neill}, J.~D. and 
	{Martin}, D.~C. and {Heckman}, T. and {Lawrence}, A. and {Norman}, C. and 
	{Narayan}, G. and {Foley}, R.~J. and {Marion}, G.~H. and {Scolnic}, D. and 
	{Chomiuk}, L. and {Soderberg}, A. and {Smith}, K. and {Kirshner}, R.~P. and 
	{Riess}, A.~G. and {Smartt}, S.~J. and {Stubbs}, C.~W. and {Tonry}, J.~L. and 
	{Wood-Vasey}, W.~M. and {Burgett}, W.~S. and {Chambers}, K.~C. and 
	{Grav}, T. and {Heasley}, J.~N. and {Kaiser}, N. and {Kudritzki}, R.-P. and 
	{Magnier}, E.~A. and {Morgan}, J.~S. and {PRICE}, P.~A.},
    title = "{An ultraviolet-optical flare from the tidal disruption of a helium-rich stellar core}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1205.0252},
 primaryClass = "astro-ph.CO",
     year = 2012,
    month = may,
   volume = 485,
    pages = {217-220},
      doi = {10.1038/nature10990},
   adsurl = {http://adsabs.harvard.edu/abs/2012Natur.485..217G},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Maksym14,
   author = {{Maksym}, W.~P. and {Lin}, D. and {Irwin}, J.~A.},
    title = "{RBS 1032: A Tidal Disruption Event in Another Dwarf Galaxy?}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1407.2928},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: dwarf, galaxies: nuclei, X-rays: bursts, X-rays: individual: RBS 1032},
     year = 2014,
    month = sep,
   volume = 792,
      eid = {L29},
    pages = {L29},
      doi = {10.1088/2041-8205/792/2/L29},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...792L..29M},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{McConnell13a,
   author = {{McConnell}, N.~J. and {Chen}, S.-F.~S. and {Ma}, C.-P. and 
	{Greene}, J.~E. and {Lauer}, T.~R. and {Gebhardt}, K.},
    title = "{The Effect of Spatial Gradients in Stellar Mass-to-light Ratio on Black Hole Mass Measurements}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1303.4393},
 keywords = {galaxies: kinematics and dynamics},
     year = 2013,
    month = may,
   volume = 768,
      eid = {L21},
    pages = {L21},
      doi = {10.1088/2041-8205/768/1/L21},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...768L..21M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{McConnell13b,
   author = {{McConnell}, N.~J. and {Ma}, C.-P.},
    title = "{Revisiting the Scaling Relations of Black Hole Masses and Host Galaxy Properties}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1211.2816},
 keywords = {galaxies: nuclei, galaxies: statistics},
     year = 2013,
    month = feb,
   volume = 764,
      eid = {184},
    pages = {184},
      doi = {10.1088/0004-637X/764/2/184},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...764..184M},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Graham14a,
   author = {{Graham}, A.~W. and {Scott}, N. and {Schombert}, J.},
    title = "{Super-massive black hole mass scaling relations}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1411.1438},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2014,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1411.1438G},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}


@ARTICLE{Graham14b,
   author = {{Graham}, A.~W.},
    title = "{Black hole and nuclear cluster scaling relations: M\_bh \~{} M\_nc\^{}$\{$2.7+/-0.7$\}$}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1412.5715},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2014,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1412.5715G},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Verolme02,
   author = {{Verolme}, E.~K. and {Cappellari}, M. and {Copin}, Y. and {van der Marel}, R.~P. and 
	{Bacon}, R. and {Bureau}, M. and {Davies}, R.~L. and {Miller}, B.~M. and 
	{de Zeeuw}, P.~T.},
    title = "{A SAURON STUDY of M32: measuring the intrinsic flattening and the central black hole mass}",
  journal = {\mnras},
   eprint = {astro-ph/0201086},
 keywords = {methods: DATA ANALYSIS, techniques: spectroscopic, galaxies: elliptical and lenticular, cD, galaxies: individual: M32, galaxies: kinematics and dynamics, galaxies: structure},
     year = 2002,
    month = sep,
   volume = 335,
    pages = {517-525},
      doi = {10.1046/j.1365-8711.2002.05664.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.335..517V},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}


@ARTICLE{Gebhardt01,
   author = {{Gebhardt}, K. and {Lauer}, T.~R. and {Kormendy}, J. and {Pinkney}, J. and 
	{Bower}, G.~A. and {Green}, R. and {Gull}, T. and {Hutchings}, J.~B. and 
	{Kaiser}, M.~E. and {Nelson}, C.~H. and {Richstone}, D. and 
	{Weistrop}, D.},
    title = "{M33: A Galaxy with No Supermassive Black Hole}",
  journal = {\aj},
   eprint = {astro-ph/0107135},
 keywords = {Galaxies: General, Galaxies: Nuclei},
     year = 2001,
    month = nov,
   volume = 122,
    pages = {2469-2476},
      doi = {10.1086/323481},
   adsurl = {http://adsabs.harvard.edu/abs/2001AJ....122.2469G},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Denbrok15,
   author = {{den Brok}, M. and {Seth}, A.~C. and {Barth}, A.~J. and {Carson}, D.~J. and 
	{Neumayer}, N. and {Cappellari}, M. and {Debattista}, V.~P. and 
	{Ho}, L.~C. and {Hood}, C.~E. and {McDermid}, R.~M.},
    title = "{Measuring the mass of the central black hole in the bulgeless galaxy NGC 4395 from gas dynamical modeling}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1507.04358},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2015,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150704358D},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Yuan14,
   author = {{Yuan}, W. and {Zhou}, H. and {Dou}, L. and {Dong}, X.-B. and 
	{Fan}, X. and {Wang}, T.-G.},
    title = "{Chandra and MMT Observations of Low-mass Black Hole ACTIVE Galactic Nuclei Accreting at Low RATES in Dwarf Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1401.5331},
 keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, X-rays: galaxies},
     year = 2014,
    month = feb,
   volume = 782,
      eid = {55},
    pages = {55},
      doi = {10.1088/0004-637X/782/1/55},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...782...55Y},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Lu15,
   author = {{Lu}, Z. and {Mo}, H.~J.},
    title = "{Classical Bulges, Supermassive Black Holes, and AGN Feedback: Extension to Low-mass Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1407.4382},
 keywords = {galaxies: evolution, galaxies: formation},
     year = 2015,
    month = apr,
   volume = 802,
      eid = {110},
    pages = {110},
      doi = {10.1088/0004-637X/802/2/110},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...802..110L},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Dong12,
   author = {{Dong}, X.-B. and {Ho}, L.~C. and {Yuan}, W. and {Wang}, T.-G. and 
	{Fan}, X. and {Zhou}, H. and {Jiang}, N.},
    title = "{A Uniformly Selected SAMPLE of Low-mass Black Holes in Seyfert 1 Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1206.3843},
 keywords = {galaxies: ACTIVE, galaxies: nuclei, galaxies: Seyfert},
     year = 2012,
    month = aug,
   volume = 755,
      eid = {167},
    pages = {167},
      doi = {10.1088/0004-637X/755/2/167},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...755..167D},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Ho12,
   author = {{Ho}, L.~C. and {Kim}, M. and {Terashima}, Y.},
    title = "{The Low-mass, Highly Accreting Black Hole Associated with the ACTIVE Galactic Nucleus 2XMM J123103.2+110648}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1210.0440},
 keywords = {black hole physics, galaxies: ACTIVE, galaxies: nuclei, galaxies: Seyfert},
     year = 2012,
    month = nov,
   volume = 759,
      eid = {L16},
    pages = {L16},
      doi = {10.1088/2041-8205/759/1/L16},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...759L..16H},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Barth09,
   author = {{Barth}, A.~J. and {Strigari}, L.~E. and {Bentz}, M.~C. and 
	{Greene}, J.~E. and {Ho}, L.~C.},
    title = "{Dynamical Constraints on the Masses of the Nuclear Star Cluster and Black Hole in the Late-Type Spiral Galaxy NGC 3621}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0809.1066},
 keywords = {galaxies: ACTIVE, galaxies: individual: NGC 3621, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: spiral},
     year = 2009,
    month = jan,
   volume = 690,
    pages = {1031-1044},
      doi = {10.1088/0004-637X/690/1/1031},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690.1031B},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Do13,
   author = {{Do}, T. and {Martinez}, G.~D. and {Yelda}, S. and {Ghez}, A. and 
	{Bullock}, J. and {Kaplinghat}, M. and {Lu}, J.~R. and {Peter}, A.~H.~G. and 
	{Phifer}, K.},
    title = "{Three-dimensional Stellar Kinematics at the Galactic Center: Measuring the Nuclear Star Cluster Spatial Density Profile, Black Hole Mass, and Distance}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1311.0886},
 keywords = {Galaxy: center, stars: kinematics and dynamics, stars: late-type, techniques: high angular resolution, techniques: spectroscopic},
     year = 2013,
    month = dec,
   volume = 779,
      eid = {L6},
    pages = {L6},
      doi = {10.1088/2041-8205/779/1/L6},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...779L...6D},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Naiman15,
   author = {{Naiman}, J.~P. and {Ramirez-Ruiz}, E. and {Debuhr}, J. and 
	{Ma}, C.-P.},
    title = "{The Role of Nuclear Star Clusters in Enhancing Supermassive Black Hole Feeding RATES During Galaxy Mergers}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1410.7381},
 keywords = {accretion, accretion disks, galaxies: ACTIVE, galaxies: nuclei},
     year = 2015,
    month = apr,
   volume = 803,
      eid = {81},
    pages = {81},
      doi = {10.1088/0004-637X/803/2/81},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...803...81N},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Matthews99,
   author = {{Matthews}, L.~D. and {Gallagher}, III, J.~S. and {Krist}, J.~E. and 
	{Watson}, A.~M. and {Burrows}, C.~J. and {Griffiths}, R.~E. and 
	{Hester}, J.~J. and {Trauger}, J.~T. and {Ballester}, G.~E. and 
	{Clarke}, J.~T. and {Crisp}, D. and {Evans}, R.~W. and {Hoessel}, J.~G. and 
	{Holtzman}, J.~A. and {Mould}, J.~R. and {Scowen}, P.~A. and 
	{Stapelfeldt}, K.~R. and {Westphal}, J.~A.},
    title = "{WFPC2 Observations of Compact Star Cluster Nuclei in Low-Luminosity Spiral Galaxies}",
  journal = {\aj},
   eprint = {astro-ph/9904205},
 keywords = {GALAXIES: ACTIVE, GALAXIES: NUCLEI, GALAXIES: SPIRAL},
     year = 1999,
    month = jul,
   volume = 118,
    pages = {208-235},
      doi = {10.1086/300909},
   adsurl = {http://adsabs.harvard.edu/abs/1999AJ....118..208M},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Walcher05,
   author = {{Walcher}, C.~J. and {van der Marel}, R.~P. and {McLaughlin}, D. and 
	{Rix}, H.-W. and {B{\"o}ker}, T. and {H{\"a}ring}, N. and {Ho}, L.~C. and 
	{Sarzi}, M. and {Shields}, J.~C.},
    title = "{Masses of Star Clusters in the Nuclei of Bulgeless Spiral Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/0409216},
 keywords = {Galaxies: Nuclei, Galaxies: Spiral, Galaxies: Star Clusters, Galaxies: Structure},
     year = 2005,
    month = jan,
   volume = 618,
    pages = {237-246},
      doi = {10.1086/425977},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...618..237W},
  adsnote = {Provided by the SAO/NASA Astrophysics DATA System}
}

@ARTICLE{Baldassare15,
   author = {{Baldassare}, V.~F. and {Reines}, A.~E. and {Gallo}, E. and 
	{Greene}, J.~E.},
    title = "{A {\sim}50,000 M$_{⊙}$ Solar Mass Black Hole in the Nucleus of RGG 118}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1506.07531},
 keywords = {galaxies: ACTIVE, galaxies: dwarf, quasars: supermassive black holes},
     year = 2015,
    month = aug,
   volume = 809,
      eid = {L14},
    pages = {L14},
      doi = {10.1088/2041-8205/809/1/L14},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...809L..14B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reines15,
   author = {{Reines}, A.~E. and {Volonteri}, M.},
    title = "{Relations Between Central Black Hole Mass and Total Galaxy Stellar Mass in the LOCAL Universe}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1508.06274},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2015,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv150806274R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reines14,
   author = {{Reines}, A.~E. and {Plotkin}, R.~M. and {Russell}, T.~D. and 
	{Mezcua}, M. and {Condon}, J.~J. and {Sivakoff}, G.~R. and {Johnson}, K.~E.
	},
    title = "{A Candidate Massive Black Hole in the Low-metallicity Dwarf Galaxy Pair Mrk 709}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1405.0278},
 keywords = {galaxies: active, galaxies: dwarf, galaxies: individual: Mrk 709, galaxies: nuclei},
     year = 2014,
    month = jun,
   volume = 787,
      eid = {L30},
    pages = {L30},
      doi = {10.1088/2041-8205/787/2/L30},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...787L..30R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Conroy13,
   author = {{Conroy}, C.},
    title = "{Modeling the Panchromatic Spectral Energy Distributions of Galaxies}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1301.7095},
     year = 2013,
    month = aug,
   volume = 51,
    pages = {393-455},
      doi = {10.1146/annurev-astro-082812-141017},
   adsurl = {http://adsabs.harvard.edu/abs/2013ARA%26A..51..393C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Osterbrock89,
   author = {{Osterbrock}, D.~E.},
    title = "{Book-Review - Astrophysics of Gaseous Nebulae and Active Galactic Nuclei}",
  journal = {\skytel},
     year = 1989,
    month = nov,
   volume = 78,
    pages = {491},
   adsurl = {http://adsabs.harvard.edu/abs/1989S%26T....78..491O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Greene05,
   author = {{Greene}, J.~E. and {Ho}, L.~C.},
    title = "{Estimating Black Hole Masses in Active Galaxies Using the H{$\alpha$} Emission Line}",
  journal = {\apj},
   eprint = {astro-ph/0508335},
 keywords = {Galaxies: Active, Galaxies: Jets, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Quasars: General},
     year = 2005,
    month = sep,
   volume = 630,
    pages = {122-129},
      doi = {10.1086/431897},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...630..122G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Panessa06,
   author = {{Panessa}, F. and {Bassani}, L. and {Cappi}, M. and {Dadina}, M. and 
	{Barcons}, X. and {Carrera}, F.~J. and {Ho}, L.~C. and {Iwasawa}, K.
	},
    title = "{On the X-ray, optical emission line and black hole mass properties of local Seyfert galaxies}",
  journal = {\aap},
   eprint = {astro-ph/0605236},
 keywords = {accretion, accretion disks, X-rays: galaxies, galaxies: Seyfert, galaxies: nuclei},
     year = 2006,
    month = aug,
   volume = 455,
    pages = {173-185},
      doi = {10.1051/0004-6361:20064894},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...455..173P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Merloni03,
   author = {{Merloni}, A. and {Heinz}, S. and {di Matteo}, T.},
    title = "{A Fundamental Plane of black hole activity}",
  journal = {\mnras},
   eprint = {astro-ph/0305261},
 keywords = {accretion, accretion discs, black hole physics, galaxies: active, radio continuum: general, X-rays: binaries, X-rays: general},
     year = 2003,
    month = nov,
   volume = 345,
    pages = {1057-1076},
      doi = {10.1046/j.1365-2966.2003.07017.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.345.1057M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Falcke04,
   author = {{Falcke}, H. and {K{\"o}rding}, E. and {Markoff}, S.},
    title = "{A scheme to unify low-power accreting black holes. Jet-dominated accretion flows and the radio/X-ray correlation}",
  journal = {\aap},
   eprint = {astro-ph/0305335},
 keywords = {X-rays: binaries, radiation mechanisms: non-thermal, stars: winds, outflows, black hole physics, accretion, accretion disks},
     year = 2004,
    month = feb,
   volume = 414,
    pages = {895-903},
      doi = {10.1051/0004-6361:20031683},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...414..895F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kording06,
   author = {{K{\"o}rding}, E. and {Falcke}, H. and {Corbel}, S.},
    title = "{Refining the fundamental plane of accreting black holes}",
  journal = {\aap},
   eprint = {astro-ph/0603117},
 keywords = {X-rays: binaries, galaxies: active, radiation mechanisms: non-thermal, stars: winds, outflows, black hole physics, accretion, accretion disks},
     year = 2006,
    month = sep,
   volume = 456,
    pages = {439-450},
      doi = {10.1051/0004-6361:20054144},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...456..439K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kennicutt98a,
   author = {{Kennicutt}, Jr., R.~C.},
    title = "{Star Formation in Galaxies Along the Hubble Sequence}",
  journal = {\araa},
   eprint = {astro-ph/9807187},
     year = 1998,
   volume = 36,
    pages = {189-232},
      doi = {10.1146/annurev.astro.36.1.189},
   adsurl = {http://adsabs.harvard.edu/abs/1998ARA%26A..36..189K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kennicutt98b,
   author = {{Kennicutt}, Jr., R.~C.},
    title = "{The Global Schmidt Law in Star-forming Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/9712213},
 keywords = {GALAXIES: EVOLUTION, GALAXIES: ISM, GALAXIES: SPIRAL, GALAXIES: STELLAR CONTENT, GALAXIES: STARBURST, STARS: FORMATION, Galaxies: Evolution, Galaxies: ISM, Galaxies: Spiral, Galaxies: Starburst, Galaxies: Stellar Content, Stars: Formation},
     year = 1998,
    month = may,
   volume = 498,
    pages = {541-552},
      doi = {10.1086/305588},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...498..541K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kewley06,
   author = {{Kewley}, L.~J. and {Groves}, B. and {Kauffmann}, G. and {Heckman}, T.
	},
    title = "{The host galaxies and classification of active galactic nuclei}",
  journal = {\mnras},
   eprint = {astro-ph/0605681},
 keywords = {galaxies: active, galaxies: Seyfert, galaxies: starburst},
     year = 2006,
    month = nov,
   volume = 372,
    pages = {961-976},
      doi = {10.1111/j.1365-2966.2006.10859.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.372..961K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Murphy11,
   author = {{Murphy}, E.~J. and {Condon}, J.~J. and {Schinnerer}, E. and 
	{Kennicutt}, R.~C. and {Calzetti}, D. and {Armus}, L. and {Helou}, G. and 
	{Turner}, J.~L. and {Aniano}, G. and {Beir{\~a}o}, P. and {Bolatto}, A.~D. and 
	{Brandl}, B.~R. and {Croxall}, K.~V. and {Dale}, D.~A. and {Donovan Meyer}, J.~L. and 
	{Draine}, B.~T. and {Engelbracht}, C. and {Hunt}, L.~K. and 
	{Hao}, C.-N. and {Koda}, J. and {Roussel}, H. and {Skibba}, R. and 
	{Smith}, J.-D.~T.},
    title = "{Calibrating Extinction-free Star Formation Rate Diagnostics with 33 GHz Free-free Emission in NGC 6946}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1105.4877},
 keywords = {cosmic rays, galaxies: individual: NGC 6946, H II regions, infrared: general, radio continuum: general, stars: formation},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {67},
    pages = {67},
      doi = {10.1088/0004-637X/737/2/67},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737...67M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bell03,
   author = {{Bell}, E.~F. and {McIntosh}, D.~H. and {Katz}, N. and {Weinberg}, M.~D.
	},
    title = "{The Optical and Near-Infrared Properties of Galaxies. I. Luminosity and Stellar Mass Functions}",
  journal = {\apjs},
   eprint = {astro-ph/0302543},
 kceywords = {Galaxies: Evolution, Galaxies: General, Galaxies: Luminosity Function, Mass Function, Galaxies: Stellar Content},
     year = 2003,
    month = dec,
   volume = 149,
    pages = {289-312},
      doi = {10.1086/378847},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJS..149..289B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bell01,
   author = {{Bell}, E.~F. and {de Jong}, R.~S.},
    title = "{Stellar Mass-to-Light Ratios and the Tully-Fisher Relation}",
  journal = {\apj},
   eprint = {astro-ph/0011493},
 keywords = {ISM: Dust, Extinction, Galaxies: Evolution, Galaxies: Kinematics and Dynamics, Galaxies: Spiral, Galaxies: Stellar Content},
     year = 2001,
    month = mar,
   volume = 550,
    pages = {212-229},
      doi = {10.1086/319728},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...550..212B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Emsellem94a,
   author = {{Emsellem}, E. and {Monnet}, G. and {Bacon}, R.},
    title = "{The multi-gaussian expansion method: a tool for building realistic photometric and kinematical models of stellar systems I. The formalism}",
  journal = {\aap},
 keywords = {GALAXIES: STRUCTURE, GALAXIES: KINEMATICS AND DYNAMICS, TECHNIQUES: IMAGE PROCESSING, CELESTIAL MECHANICS, STELLAR DYNAMICS},
     year = 1994,
    month = may,
   volume = 285,
    pages = {723-738},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...285..723E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Emsellem94b,
   author = {{Emsellem}, E. and {Monnet}, G. and {Bacon}, R. and {Nieto}, J.-L.
	},
    title = "{The multi-gaussian expansion method: a tool for building realistic photometric and kinematical models of stellar systems II. Application to the central region of the Sombrero Galaxy (NGC 4594)}",
  journal = {\aap},
 keywords = {GALAXIES: INDIVIDUAL: NGC 4594, GALAXIES: STRUCTURE, GALAXIES: LUMINOSITY FUNCTION, MASS FUNCTION, GALAXIES: KINEMATICS AND DYNAMICS OF, GALAXIES: NUCLEI, IMAGE PROCESSING},
     year = 1994,
    month = may,
   volume = 285,
    pages = {739-750},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...285..739E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari04,
   author = {{Cappellari}, M. and {Emsellem}, E.},
    title = "{Parametric Recovery of Line-of-Sight Velocity Distributions from Absorption-Line Spectra of Galaxies via Penalized Likelihood}",
  journal = {\pasp},
   eprint = {astro-ph/0312201},
 keywords = {Galaxies: Individual: NGC Number: NGC 3384, Galaxies: Kinematics and Dynamics, line: profiles, Methods: Numerical},
     year = 2004,
    month = feb,
   volume = 116,
    pages = {138-147},
      doi = {10.1086/381875},
   adsurl = {http://adsabs.harvard.edu/abs/2004PASP..116..138C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari15,
   author = {{Cappellari}, M. and {Romanowsky}, A.~J. and {Brodie}, J.~P. and 
	{Forbes}, D.~A. and {Strader}, J. and {Foster}, C. and {Kartha}, S.~S. and 
	{Pastorello}, N. and {Pota}, V. and {Spitler}, L.~R. and {Usher}, C. and 
	{Arnold}, J.~A.},
    title = "{Small Scatter and Nearly Isothermal Mass Profiles to Four Half-light Radii from Two-dimensional Stellar Dynamics of Early-type Galaxies}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1504.00075},
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: formation, galaxies: kinematics and dynamics, galaxies: structure},
     year = 2015,
    month = may,
   volume = 804,
      eid = {L21},
    pages = {L21},
      doi = {10.1088/2041-8205/804/1/L21},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...804L..21C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari12,
   author = {{Cappellari}, M. and {McDermid}, R.~M. and {Alatalo}, K. and 
	{Blitz}, L. and {Bois}, M. and {Bournaud}, F. and {Bureau}, M. and 
	{Crocker}, A.~F. and {Davies}, R.~L. and {Davis}, T.~A. and 
	{de Zeeuw}, P.~T. and {Duc}, P.-A. and {Emsellem}, E. and {Khochfar}, S. and 
	{Krajnovi{\'c}}, D. and {Kuntschner}, H. and {Lablanche}, P.-Y. and 
	{Morganti}, R. and {Naab}, T. and {Oosterloo}, T. and {Sarzi}, M. and 
	{Scott}, N. and {Serra}, P. and {Weijmans}, A.-M. and {Young}, L.~M.
	},
    title = "{Systematic variation of the stellar initial mass function in early-type galaxies}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1202.3308},
 primaryClass = "astro-ph.CO",
     year = 2012,
    month = apr,
   volume = 484,
    pages = {485-488},
      doi = {10.1038/nature10972},
   adsurl = {http://adsabs.harvard.edu/abs/2012Natur.484..485C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Conroy12,
   author = {{Conroy}, C. and {van Dokkum}, P.~G.},
    title = "{The Stellar Initial Mass Function in Early-type Galaxies From Absorption Line Spectroscopy. II. Results}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1205.6473},
 keywords = {galaxies: abundances, galaxies: elliptical and lenticular, cD, galaxies: stellar content},
     year = 2012,
    month = nov,
   volume = 760,
      eid = {71},
    pages = {71},
      doi = {10.1088/0004-637X/760/1/71},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...760...71C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Cappellari13b,
   author = {{Cappellari}, M. and {McDermid}, R.~M. and {Alatalo}, K. and 
	{Blitz}, L. and {Bois}, M. and {Bournaud}, F. and {Bureau}, M. and 
	{Crocker}, A.~F. and {Davies}, R.~L. and {Davis}, T.~A. and 
	{de Zeeuw}, P.~T. and {Duc}, P.-A. and {Emsellem}, E. and {Khochfar}, S. and 
	{Krajnovi{\'c}}, D. and {Kuntschner}, H. and {Morganti}, R. and 
	{Naab}, T. and {Oosterloo}, T. and {Sarzi}, M. and {Scott}, N. and 
	{Serra}, P. and {Weijmans}, A.-M. and {Young}, L.~M.},
    title = "{The ATLAS$^{3D}$ project - XX. Mass-size and mass-{$\sigma$} distributions of early-type galaxies: bulge fraction drives kinematics, mass-to-light ratio, molecular gas fraction and stellar initial mass function}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1208.3523},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, galaxies: structure},
     year = 2013,
    month = jul,
   volume = 432,
    pages = {1862-1893},
      doi = {10.1093/mnras/stt644},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.432.1862C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari12c,
   author = {{Cappellari}, M.},
    title = "{Effect of Environment on Galaxies' Mass-Size Distribution: Unveiling the Transition from outside-in to inside-out Evolution}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1309.1136},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: clusters: individual: Abell 1656, galaxies: evolution, galaxies: formation, galaxies: structure},
     year = 2013,
    month = nov,
   volume = 778,
      eid = {L2},
    pages = {L2},
      doi = {10.1088/2041-8205/778/1/L2},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...778L...2C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari12a,
   author = {{Cappellari}, M. and {Scott}, N. and {Alatalo}, K. and {Blitz}, L. and 
	{Bois}, M. and {Bournaud}, F. and {Bureau}, M. and {Crocker}, A.~F. and 
	{Davies}, R.~L. and {Davis}, T.~A. and {de Zeeuw}, P.~T. and 
	{Duc}, P.-A. and {Emsellem}, E. and {Khochfar}, S. and {Krajnovi{\'c}}, D. and 
	{Kuntschner}, H. and {McDermid}, R.~M. and {Morganti}, R. and 
	{Naab}, T. and {Oosterloo}, T. and {Sarzi}, M. and {Serra}, P. and 
	{Weijmans}, A.-M. and {Young}, L.~M.},
    title = "{The ATLAS$^{3D}$ project - XV. Benchmark for early-type galaxies scaling relations from 260 dynamical models: mass-to-light ratio, dark matter, Fundamental Plane and Mass Plane}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1208.3522},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, galaxies: structure},
     year = 2013,
    month = jul,
   volume = 432,
    pages = {1709-1741},
      doi = {10.1093/mnras/stt562},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.432.1709C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Greene12,
   author = {{Greene}, J.~E.},
    title = "{Low-mass black holes as the remnants of primordial black hole formation}",
  journal = {Nature Communications},
archivePrefix = "arXiv",
   eprint = {1211.7082},
     year = 2012,
    month = dec,
   volume = 3,
      eid = {1304},
    pages = {1304},
      doi = {10.1038/ncomms2314},
   adsurl = {http://adsabs.harvard.edu/abs/2012NatCo...3E1304G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lutzgendorf11,
   author = {{L{\"u}tzgendorf}, N. and {Kissler-Patig}, M. and {Noyola}, E. and 
	{Jalali}, B. and {de Zeeuw}, P.~T. and {Gebhardt}, K. and {Baumgardt}, H.
	},
    title = "{Kinematic signature of an intermediate-mass black hole in the globular cluster NGC 6388}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1107.4243},
 keywords = {black hole physics, globular clusters: individual: NGC 6388, stars: kinematics and dynamics},
     year = 2011,
    month = sep,
   volume = 533,
      eid = {A36},
    pages = {A36},
      doi = {10.1051/0004-6361/201116618},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...533A..36L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lutzgendorf13b,
   author = {{L{\"u}tzgendorf}, N. and {Kissler-Patig}, M. and {Neumayer}, N. and 
	{Baumgardt}, H. and {Noyola}, E. and {de Zeeuw}, P.~T. and {Gebhardt}, K. and 
	{Jalali}, B. and {Feldmeier}, A.},
    title = "{M$_{•}$ - {$\sigma$}relation for intermediate-mass black holes in globular clusters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1304.7156},
 keywords = {black hole physics, stars: kinematics and dynamics},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {A26},
    pages = {A26},
      doi = {10.1051/0004-6361/201321183},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555A..26L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lutzgendorf13a,
   author = {{L{\"u}tzgendorf}, N. and {Kissler-Patig}, M. and {Gebhardt}, K. and 
	{Baumgardt}, H. and {Noyola}, E. and {de Zeeuw}, P.~T. and {Neumayer}, N. and 
	{Jalali}, B. and {Feldmeier}, A.},
    title = "{Limits on intermediate-mass black holes in six Galactic globular clusters with integral-field spectroscopy}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1212.3475},
 keywords = {black hole physics, globular clusters: general, stars: kinematics and dynamics},
     year = 2013,
    month = apr,
   volume = 552,
      eid = {A49},
    pages = {A49},
      doi = {10.1051/0004-6361/201220307},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...552A..49L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lutzgendorf13c,
   author = {{L{\"u}tzgendorf}, N. and {Baumgardt}, H. and {Kruijssen}, J.~M.~D.
	},
    title = "{N-body simulations of globular clusters in tidal fields: Effects of intermediate-mass black holes}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1309.0451},
 keywords = {black hole physics, stars: kinematics and dynamics, methods: numerical, galaxies: star clusters: general},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A117},
    pages = {A117},
      doi = {10.1051/0004-6361/201321927},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...558A.117L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jalali12,
   author = {{Jalali}, B. and {Baumgardt}, H. and {Kissler-Patig}, M. and 
	{Gebhardt}, K. and {Noyola}, E. and {L{\"u}tzgendorf}, N. and 
	{de Zeeuw}, P.~T.},
    title = "{A Dynamical N-body model for the central region of {$\omega$} Centauri}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1111.5011},
 keywords = {methods: numerical, black hole physics, Galaxy: kinematics and dynamics, globular clusters: individual:{$\omega$}Centauri},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A19},
    pages = {A19},
      doi = {10.1051/0004-6361/201116923},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A..19J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jarrett03,
   author = {{Jarrett}, T.~H. and {Chester}, T. and {Cutri}, R. and {Schneider}, S.~E. and 
	{Huchra}, J.~P.},
    title = "{The 2MASS Large Galaxy Atlas}",
  journal = {\aj},
 keywords = {Atlases, Galaxies: Fundamental Parameters, Galaxies: Photometry, Galaxies: Statistics, Galaxy: Globular Clusters: General, Infrared Radiation, Surveys},
     year = 2003,
    month = feb,
   volume = 125,
    pages = {525-554},
      doi = {10.1086/345794},
   adsurl = {http://adsabs.harvard.edu/abs/2003AJ....125..525J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Williams10,
   author = {{Williams}, B.~F. and {Dalcanton}, J.~J. and {Gilbert}, K.~M. and 
	{Stilp}, A. and {Dolphin}, A. and {Seth}, A.~C. and {Weisz}, D. and 
	{Skillman}, E.},
    title = "{The Advanced Camera for Surveys Nearby Galaxy Survey Treasury. VI. The Ancient Star-forming Disk of NGC 404}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1004.5135},
 keywords = {galaxies: evolution, galaxies: individual: NGC 404, galaxies: stellar content},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {71-83},
      doi = {10.1088/0004-637X/716/1/71},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716...71W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strader11b,
   author = {{Strader}, J. and {Romanowsky}, A.~J. and {Brodie}, J.~P. and 
	{Spitler}, L.~R. and {Beasley}, M.~A. and {Arnold}, J.~A. and 
	{Tamura}, N. and {Sharples}, R.~M. and {Arimoto}, N.},
    title = "{Wide-field Precision Kinematics of the M87 Globular Cluster System}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1110.2778},
 keywords = {dark matter, galaxies: elliptical and lenticular, cD, galaxies: individual: M87, galaxies: kinematics and dynamics, galaxies: star clusters: general, globular clusters: general},
     year = 2011,
    month = dec,
   volume = 197,
      eid = {33},
    pages = {33},
      doi = {10.1088/0067-0049/197/2/33},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..197...33S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strader11a,
   author = {{Strader}, J. and {Caldwell}, N. and {Seth}, A.~C.},
    title = "{Star Clusters in M31. V. Internal Dynamical Trends: Some Troublesome, Some Reassuring}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1104.4649},
 keywords = {galaxies: individual: M31, galaxies: star clusters: general, globular clusters: general, stars: luminosity function, mass function},
     year = 2011,
    month = jul,
   volume = 142,
      eid = {8},
    pages = {8},
      doi = {10.1088/0004-6256/142/1/8},
   adsurl = {http://adsabs.harvard.edu/abs/2011AJ....142....8S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vandenBosch10,
   author = {{van den Bosch}, R.~C.~E. and {de Zeeuw}, P.~T.},
    title = "{Estimating black hole masses in triaxial galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0910.0844},
 primaryClass = "astro-ph.CO",
 keywords = {black hole physics, galaxies: elliptical and lenticular, cD, galaxies: individual: NGC 3379, galaxies: individual: M32, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: structure},
     year = 2010,
    month = jan,
   volume = 401,
    pages = {1770-1780},
      doi = {10.1111/j.1365-2966.2009.15832.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.401.1770V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vandenBosch12,
   author = {{van den Bosch}, R.~C.~E. and {Gebhardt}, K. and {G{\"u}ltekin}, K. and 
	{van de Ven}, G. and {van der Wel}, A. and {Walsh}, J.~L.},
    title = "{An over-massive black hole in the compact lenticular galaxy NGC 1277}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1211.6429},
 primaryClass = "astro-ph.CO",
     year = 2012,
    month = nov,
   volume = 491,
    pages = {729-731},
      doi = {10.1038/nature11592},
   adsurl = {http://adsabs.harvard.edu/abs/2012Natur.491..729V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Emsellem13,
   author = {{Emsellem}, E.},
    title = "{Is the black hole in NGC 1277 really overmassive?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1305.3630},
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: structure},
     year = 2013,
    month = aug,
   volume = 433,
    pages = {1862-1870},
      doi = {10.1093/mnras/stt840},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433.1862E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Walsh15,
   author = {{Walsh}, J.~L. and {van den Bosch}, R.~C.~E. and {Gebhardt}, K. and 
	{Y{\i}ld{\i}r{\i}m}, A. and {Richstone}, D.~O. and {G{\"u}ltekin}, K. and 
	{Husemann}, B.},
    title = "{A 5x10\^{}9 Solar Mass Black Hole in NGC 1277 from Adaptive Optics Spectroscopy}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1511.04455},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2015,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv151104455W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PortegiesZwart04b,
   author = {{Portegies Zwart}, S.~F. and {Baumgardt}, H. and {Hut}, P. and 
	{Makino}, J. and {McMillan}, S.~L.~W.},
    title = "{Formation of massive black holes through runaway collisions in dense young star clusters}",
  journal = {\nat},
   eprint = {astro-ph/0402622},
     year = 2004,
    month = apr,
   volume = 428,
    pages = {724-726},
      doi = {10.1038/nature02448},
   adsurl = {http://adsabs.harvard.edu/abs/2004Natur.428..724P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PortegiesZwart04a,
   author = {{Portegies Zwart}, S.~F. and {Dewi}, J. and {Maccarone}, T.},
    title = "{Intermediate mass black holes in accreting binaries: formation, evolution and observational appearance}",
  journal = {\mnras},
   eprint = {astro-ph/0408402},
 keywords = {black hole physics, binaries: close, galaxies: individual: M82, X-rays: binaries, X-rays: individual: M82 X-1},
     year = 2004,
    month = dec,
   volume = 355,
    pages = {413-423},
      doi = {10.1111/j.1365-2966.2004.08327.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.355..413P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Antonini15b,
   author = {{Antonini}, F. and {Barausse}, E. and {Silk}, J.},
    title = "{The Imprint of Massive Black Hole Mergers on the Correlation between Nuclear Star Clusters and Their Host Galaxies}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1504.04033},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: nuclei, Galaxy: center},
     year = 2015,
    month = jun,
   volume = 806,
      eid = {L8},
    pages = {L8},
      doi = {10.1088/2041-8205/806/1/L8},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...806L...8A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Antonini15a,
   author = {{Antonini}, F. and {Barausse}, E. and {Silk}, J.},
    title = "{The Coevolution of Nuclear Star Clusters, Massive Black Holes, and Their Host Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1506.02050},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: nuclei, Galaxy: center, quasars: supermassive black holes},
     year = 2015,
    month = oct,
   volume = 812,
      eid = {72},
    pages = {72},
      doi = {10.1088/0004-637X/812/1/72},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...812...72A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nayakshin09b,
   author = {{Nayakshin}, S. and {Wilkinson}, M.~I. and {King}, A.},
    title = "{Competitive feedback in galaxy formation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0907.1002},
 keywords = {accretion, accretion discs, galaxies: active, galaxies: formation},
     year = 2009,
    month = sep,
   volume = 398,
    pages = {L54-L57},
      doi = {10.1111/j.1745-3933.2009.00709.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.398L..54N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nayakshin09a,
   author = {{Nayakshin}, S. and {Cha}, S.-H. and {Hobbs}, A.},
    title = "{Dynamic Monte Carlo radiation transfer in SPH: radiation pressure force implementation}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0905.2896},
 primaryClass = "astro-ph.IM",
 keywords = {hydrodynamics , radiative transfer},
     year = 2009,
    month = aug,
   volume = 397,
    pages = {1314-1325},
      doi = {10.1111/j.1365-2966.2009.15091.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.397.1314N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Greene10,
   author = {{Greene}, J.~E. and {Peng}, C.~Y. and {Kim}, M. and {Kuo}, C.-Y. and 
	{Braatz}, J.~A. and {Impellizzeri}, C.~M.~V. and {Condon}, J.~J. and 
	{Lo}, K.~Y. and {Henkel}, C. and {Reid}, M.~J.},
    title = "{Precise Black Hole Masses from Megamaser Disks: Black Hole-Bulge Relations at Low Mass}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1007.2851},
 keywords = {galaxies: active, galaxies: bulges, galaxies: nuclei, galaxies: Seyfert},
     year = 2010,
    month = sep,
   volume = 721,
    pages = {26-45},
      doi = {10.1088/0004-637X/721/1/26},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...721...26G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Graham15,
   author = {{Graham}, A.~W. and {Scott}, N.},
    title = "{The (Black Hole)-bulge Mass Scaling Relation at Low Masses}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1412.3091},
 keywords = {black hole physics, galaxies: bulges, galaxies: fundamental parameters, galaxies: nuclei},
     year = 2015,
    month = jan,
   volume = 798,
      eid = {54},
    pages = {54},
      doi = {10.1088/0004-637X/798/1/54},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...798...54G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mieske13,
   author = {{Mieske}, S. and {Frank}, M.~J. and {Baumgardt}, H. and {L{\"u}tzgendorf}, N. and 
	{Neumayer}, N. and {Hilker}, M.},
    title = "{On central black holes in ultra-compact dwarf galaxies}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1308.1398},
 keywords = {galaxies: clusters: general, galaxies: dwarf, galaxies: star clusters: general, galaxies: nuclei, galaxies: interactions, stars: kinematics and dynamics},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A14},
    pages = {A14},
      doi = {10.1051/0004-6361/201322167},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...558A..14M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stauffer82,
   author = {{Stauffer}, J.~R.},
    title = "{A nuclear spectroscopic survey of disk galaxies. II - Galaxies with emission lines not excited by stellar photoionization}",
  journal = {\apj},
 keywords = {Astronomical Spectroscopy, Disk Galaxies, Galactic Nuclei, Seyfert Galaxies, Spectrophotometry, Active Galactic Nuclei, Active Galaxies, Emission Spectra, Photoionization, Signal To Noise Ratios},
     year = 1982,
    month = nov,
   volume = 262,
    pages = {66-80},
      doi = {10.1086/160397},
   adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...262...66S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Keel83,
   author = {{Keel}, W.~C.},
    title = "{Spectroscopic evidence for activity in the nuclei of normal spiral galaxies}",
  journal = {\apj},
 keywords = {Emission Spectra, Galactic Nuclei, H Alpha Line, Interstellar Gas, Photoionization, Spiral Galaxies, Abundance, Astronomical Models, Continuous Spectra, Data Simulation, Nonthermal Radiation, Shock Heating, Spectral Line Width, Spectrophotometry},
     year = 1983,
    month = jun,
   volume = 269,
    pages = {466-486},
      doi = {10.1086/161057},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...269..466K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tikhonov03,
   author = {{Tikhonov}, N.~A. and {Galazutdinova}, O.~A. and {Aparicio}, A.
	},
    title = "{Stellar content of NGC 404 - The nearest S0 Galaxy}",
  journal = {\aap},
 keywords = {galaxies: individual: NGC 404, galaxies: stellar content, galaxies: photometry, galaxies: distance and redshifts},
     year = 2003,
    month = apr,
   volume = 401,
    pages = {863-872},
      doi = {10.1051/0004-6361:20021819},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...401..863T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bender05,
   author = {{Bender}, R. and {Kormendy}, J. and {Bower}, G. and {Green}, R. and 
	{Thomas}, J. and {Danks}, A.~C. and {Gull}, T. and {Hutchings}, J.~B. and 
	{Joseph}, C.~L. and {Kaiser}, M.~E. and {Lauer}, T.~R. and {Nelson}, C.~H. and 
	{Richstone}, D. and {Weistrop}, D. and {Woodgate}, B.},
    title = "{HST STIS Spectroscopy of the Triple Nucleus of M31: Two Nested Disks in Keplerian Rotation around a Supermassive Black Hole}",
  journal = {\apj},
   eprint = {astro-ph/0509839},
 keywords = {Black Hole Physics, Galaxies: Individual: Messier Number: M31, Galaxies: Nuclei},
     year = 2005,
    month = sep,
   volume = 631,
    pages = {280-300},
      doi = {10.1086/432434},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...631..280B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Meyer12,
   author = {{Meyer}, F. and {Meyer-Hofmeister}, E.},
    title = "{A nova origin of the gas cloud at the Galactic center?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1208.6514},
 primaryClass = "astro-ph.SR",
 keywords = {Galaxy: center, ISM: clouds, novae, cataclysmic variables},
     year = 2012,
    month = oct,
   volume = 546,
      eid = {L2},
    pages = {L2},
      doi = {10.1051/0004-6361/201220145},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...546L...2M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Genzel10,
   author = {{Genzel}, R. and {Tacconi}, L.~J. and {Gracia-Carpio}, J. and 
	{Sternberg}, A. and {Cooper}, M.~C. and {Shapiro}, K. and {Bolatto}, A. and 
	{Bouch{\'e}}, N. and {Bournaud}, F. and {Burkert}, A. and {Combes}, F. and 
	{Comerford}, J. and {Cox}, P. and {Davis}, M. and {Schreiber}, N.~M.~F. and 
	{Garcia-Burillo}, S. and {Lutz}, D. and {Naab}, T. and {Neri}, R. and 
	{Omont}, A. and {Shapley}, A. and {Weiner}, B.},
    title = "{A study of the gas-star formation relation over cosmic time}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1003.5180},
 keywords = {stars: formation, ISM: molecules, galaxies: evolution, galaxies: ISM, galaxies: starbursts},
     year = 2010,
    month = oct,
   volume = 407,
    pages = {2091-2108},
      doi = {10.1111/j.1365-2966.2010.16969.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.407.2091G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Karachentsev02,
   author = {{Karachentsev}, I.~D. and {Sharina}, M.~E. and {Makarov}, D.~I. and 
	{Dolphin}, A.~E. and {Grebel}, E.~K. and {Geisler}, D. and {Guhathakurta}, P. and 
	{Hodge}, P.~W. and {Karachentseva}, V.~E. and {Sarajedini}, A. and 
	{Seitzer}, P.},
    title = "{The very local Hubble flow}",
  journal = {\aap},
   eprint = {astro-ph/0204507},
 keywords = {galaxies: dwarf, galaxies: distances and redshifts, galaxies: kinematics and dynamics, galaxies: Local Group},
     year = 2002,
    month = jul,
   volume = 389,
    pages = {812-824},
      doi = {10.1051/0004-6361:20020649},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...389..812K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Beii01,
   author = {{Bell}, E.~F. and {de Jong}, R.~S.},
    title = "{Stellar Mass-to-Light Ratios and the Tully-Fisher Relation}",
  journal = {\apj},
   eprint = {astro-ph/0011493},
 keywords = {ISM: Dust, Extinction, Galaxies: Evolution, Galaxies: Kinematics and Dynamics, Galaxies: Spiral, Galaxies: Stellar Content},
     year = 2001,
    month = mar,
   volume = 550,
    pages = {212-229},
      doi = {10.1086/319728},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...550..212B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zibetti09,
   author = {{Zibetti}, S. and {Charlot}, S. and {Rix}, H.-W.},
    title = "{Resolved stellar mass maps of galaxies - I. Method and implications for global mass estimates}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0904.4252},
 primaryClass = "astro-ph.CO",
 keywords = {techniques: image processing , techniques: photometric , galaxies: fundamental parameters , galaxies: general , galaxies: photometry , galaxies: stellar content},
     year = 2009,
    month = dec,
   volume = 400,
    pages = {1181-1198},
      doi = {10.1111/j.1365-2966.2009.15528.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.400.1181Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krajnovic06,
   author = {{Krajnovi{\'c}}, D. and {Cappellari}, M. and {de Zeeuw}, P.~T. and 
	{Copin}, Y.},
    title = "{Kinemetry: a generalization of photometry to the higher moments of the line-of-sight velocity distribution}",
  journal = {\mnras},
   eprint = {astro-ph/0512200},
 keywords = {methods: data analysis, techniques: photometric, techniques: spectroscopic, galaxies: kinematics and dynamics, galaxies: photometry},
     year = 2006,
    month = mar,
   volume = 366,
    pages = {787-802},
      doi = {10.1111/j.1365-2966.2005.09902.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.366..787K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Drehmer15,
   author = {{Drehmer}, D.~A. and {Storchi-Bergmann}, T. and {Ferrari}, F. and 
	{Cappellari}, M. and {Riffel}, R.~A.},
    title = "{The benchmark black hole in NGC 4258: dynamical models from high-resolution two-dimensional stellar kinematics}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1503.04540},
 keywords = {galaxies: individual: NGC 4258, galaxies: kinematics and dynamics},
     year = 2015,
    month = jun,
   volume = 450,
    pages = {128-144},
      doi = {10.1093/mnras/stv536},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.450..128D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jedrzejewski87,
   author = {{Jedrzejewski}, R.~I.},
    title = "{CCD surface photometry of elliptical galaxies. I - Observations, reduction and results}",
  journal = {\mnras},
 keywords = {Astronomical Photometry, Charge Coupled Devices, Elliptical Galaxies, Accuracy, Brightness, Data Reduction, Galactic Structure, Isophotes},
     year = 1987,
    month = jun,
   volume = 226,
    pages = {747-768},
      doi = {10.1093/mnras/226.4.747},
   adsurl = {http://adsabs.harvard.edu/abs/1987MNRAS.226..747J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Draine03,
   author = {{Draine}, B.~T.},
    title = "{Interstellar Dust Grains}",
  journal = {\araa},
   eprint = {astro-ph/0304489},
     year = 2003,
   volume = 41,
    pages = {241-289},
      doi = {10.1146/annurev.astro.41.011802.094840},
   adsurl = {http://adsabs.harvard.edu/abs/2003ARA%26A..41..241D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cardelli89,
   author = {{Cardelli}, J.~A. and {Clayton}, G.~C. and {Mathis}, J.~S.},
    title = "{The relationship between infrared, optical, and ultraviolet extinction}",
  journal = {\apj},
 keywords = {Infrared Spectra, Interstellar Extinction, Ultraviolet Spectra, Visible Spectrum, Computational Astrophysics, Interstellar Matter, Iue},
     year = 1989,
    month = oct,
   volume = 345,
    pages = {245-256},
      doi = {10.1086/167900},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...345..245C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cavanaugh97,
   author = {{Cavanaugh}, Joseph E.},
    title = "{Unifying the derivations for the Akaike and corrected Akaike information criteria}",
  journal = {Statistics \& Probability Letters},
 keywords = {AIC; AICc; Information theory; Kullback-Leibler information; Model selection},
     year = 1997,
    month = apr,
   volume = 33,
    pages = {201-208},
      doi = {10.1016/S0167-7152(96)00128-9},
   adsurl = {http://www.sciencedirect.com/science/article/pii/S0167715296001289#},
  adsnote = {http://www.sciencedirect.com/science/journal/01677152}
}

@INBOOK{Burnham02,
   author = {{Burnham}, K. P. and {Anderson}, D. R.},
    booktitle = "{Model Selection and Multimodel Inference: A Practical Information-Theoretic Approach (2nd ed.)}",
    title = "{Model Selection and Multimodel Inference: A Practical Information-Theoretic Approach (2nd ed.)}",
  publisher = {Springer-Verlag},
 keywords = {AIC; AICc; Information theory; Kullback-Leibler information; Model selection},
     year = 2002,
  pages = {100}

}

@ARTICLE{Nyland16,
   author = {{Nyland}, K. and {Young}, L. M. and {Wrobel}, J. M. and {Nguyen}, D. D. and {Seth}, A. C. and {Morganti,} R. and {Paragi} Zsolt},
    title = "{Resolved Radio Emission in the Center of NGC 404}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1305.2873},
 keywords = {galaxies: elliptical and lenticular -- galaxies: active -- galaxies: nuclei -- radio continuum: galaxies},
     year = 2016,
    month = feb,
   volume = 438,
    pages = {1483-1499},
      doi = {10.1093/mnras/stt2282},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.1483S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Georgiev16,
   author = {{Georgiev}, I.~Y. and {B{\"o}ker}, T. and {Leigh}, N. and {L{\"u}tzgendorf}, N. and 
	{Neumayer}, N.},
    title = "{Masses and Scaling Relations for Nuclear Star Clusters, and their Coexistence with Central Black Holes}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1601.02613},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160102613G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Saglia16,
   author = {{Saglia}, R.~P. and {Opitsch}, M. and {Erwin}, P. and {Thomas}, J. and 
	{Beifiori}, A. and {Fabricius}, M. and {Mazzalay}, X. and {Nowak}, N. and 
	{Rusli}, S.~P. and {Bender}, R.},
    title = "{The SINFONI Black Hole Survey: The Black Hole Fundamental Plane revisited and the paths of (co-) evolution of supermassive black holes and bulges}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1601.00974},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160100974S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Neumayer12,
   author = {{Neumayer}, N. and {Walcher}, C.~J.},
    title = "{Are Nuclear Star Clusters the Precursors of Massive Black Holes?}",
  journal = {Advances in Astronomy},
archivePrefix = "arXiv",
   eprint = {1201.4950},
     year = 2012,
   volume = 2012,
      eid = {709038},
    pages = {709038},
      doi = {10.1155/2012/709038},
   adsurl = {http://adsabs.harvard.edu/abs/2012AdAst2012E..15N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari03,
   author = {{Cappellari}, M. and {Copin}, Y.},
    title = "{Adaptive spatial binning of integral-field spectroscopic data using Voronoi tessellations}",
  journal = {\mnras},
   eprint = {astro-ph/0302262},
 keywords = {methods: data analysis, techniques: photometric, techniques: spectroscopic},
     year = 2003,
    month = jun,
   volume = 342,
    pages = {345-354},
      doi = {10.1046/j.1365-8711.2003.06541.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.342..345C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Singh13,
   author = {{Singh}, R. and {van de Ven}, G. and {Jahnke}, K. and {Lyubenova}, M. and 
	{Falc{\'o}n-Barroso}, J. and {Alves}, J. and {Cid Fernandes}, R. and 
	{Galbany}, L. and {Garc{\'{\i}}a-Benito}, R. and {Husemann}, B. and 
	{Kennicutt}, R.~C. and {Marino}, R.~A. and {M{\'a}rquez}, I. and 
	{Masegosa}, J. and {Mast}, D. and {Pasquali}, A. and {S{\'a}nchez}, S.~F. and 
	{Walcher}, J. and {Wild}, V. and {Wisotzki}, L. and {Ziegler}, B.
	},
    title = "{The nature of LINER galaxies:. Ubiquitous hot old stars and rare accreting black holes}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1308.4271},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: active, galaxies: ISM, galaxies: nuclei, stars: AGB and post-AGB},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A43},
    pages = {A43},
      doi = {10.1051/0004-6361/201322062},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...558A..43S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Jordi05,
   author = {{Jordi}, C. and {H{\o}g}, E.},
    title = "{Photometric System Design and Performances}",
 keywords = {Gaia, Photometry, Galactic astronomy, Stellar classification},
booktitle = {The Three-Dimensional Universe with Gaia},
     year = 2005,
   series = {ESA Special Publication},
   volume = 576,
   editor = {{Turon}, C. and {O'Flaherty}, K.~S. and {Perryman}, M.~A.~C.
	},
    month = jan,
    pages = {43},
   adsurl = {http://adsabs.harvard.edu/abs/2005ESASP.576...43J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Vazdekis10a,
   author = {{Vazdekis}, A. and {S{\'a}nchez-Bl{\'a}zquez}, P. and {Falc{\'o}n-Barroso}, J. and 
	{Cenarro}, A.~J. and {Beasley}, M.~A. and {Cardiel}, N. and 
	{Gorgas}, J. and {Peletier}, R.},
    title = "{MILES SSP Models}",
 keywords = {galaxies: abundances, galaxies: star clusters galaxies: dwarf galaxies: elliptical and lenticular, cD galaxies: evolution galaxies: stellar content},
booktitle = {Stellar Populations - Planning for the Next Decade},
     year = 2010,
   series = {IAU Symposium},
   volume = 262,
   editor = {{Bruzual}, G.~R. and {Charlot}, S.},
    month = apr,
    pages = {65-68},
      doi = {10.1017/S174392131000253X},
   adsurl = {http://adsabs.harvard.edu/abs/2010IAUS..262...65V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vazdekis10b,
   author = {{Vazdekis}, A. and {S{\'a}nchez-Bl{\'a}zquez}, P. and {Falc{\'o}n-Barroso}, J. and 
	{Cenarro}, A.~J. and {Beasley}, M.~A. and {Cardiel}, N. and 
	{Gorgas}, J. and {Peletier}, R.~F.},
    title = "{Evolutionary stellar population synthesis with MILES - I. The base models and a new line index system}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1004.4439},
 primaryClass = "astro-ph.CO",
 keywords = {globular clusters: general, galaxies: abundances, galaxies: elliptical and lenticular, cD, galaxies: stellar content},
     year = 2010,
    month = jun,
   volume = 404,
    pages = {1639-1671},
      doi = {10.1111/j.1365-2966.2010.16407.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.404.1639V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Calzetti00,
   author = {{Calzetti}, D. and {Armus}, L. and {Bohlin}, R.~C. and {Kinney}, A.~L. and 
	{Koornneef}, J. and {Storchi-Bergmann}, T.},
    title = "{The Dust Content and Opacity of Actively Star-forming Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/9911459},
 keywords = {GALAXIES: STARBURST, INFRARED: GALAXIES, INFRARED: ISM: CONTINUUM, ISM: DUST, EXTINCTION},
     year = 2000,
    month = apr,
   volume = 533,
    pages = {682-695},
      doi = {10.1086/308692},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...533..682C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Taylor11,
   author = {{Taylor}, E.~N. and {Hopkins}, A.~M. and {Baldry}, I.~K. and 
	{Brown}, M.~J.~I. and {Driver}, S.~P. and {Kelvin}, L.~S. and 
	{Hill}, D.~T. and {Robotham}, A.~S.~G. and {Bland-Hawthorn}, J. and 
	{Jones}, D.~H. and {Sharp}, R.~G. and {Thomas}, D. and {Liske}, J. and 
	{Loveday}, J. and {Norberg}, P. and {Peacock}, J.~A. and {Bamford}, S.~P. and 
	{Brough}, S. and {Colless}, M. and {Cameron}, E. and {Conselice}, C.~J. and 
	{Croom}, S.~M. and {Frenk}, C.~S. and {Gunawardhana}, M. and 
	{Kuijken}, K. and {Nichol}, R.~C. and {Parkinson}, H.~R. and 
	{Phillipps}, S. and {Pimbblet}, K.~A. and {Popescu}, C.~C. and 
	{Prescott}, M. and {Sutherland}, W.~J. and {Tuffs}, R.~J. and 
	{van Kampen}, E. and {Wijesinghe}, D.},
    title = "{Galaxy And Mass Assembly (GAMA): stellar mass estimates}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1108.0635},
 primaryClass = "astro-ph.CO",
 keywords = {catalogues, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: stellar content},
     year = 2011,
    month = dec,
   volume = 418,
    pages = {1587-1620},
      doi = {10.1111/j.1365-2966.2011.19536.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.418.1587T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Roediger15,
   author = {{Roediger}, J.~C. and {Courteau}, S.},
    title = "{On the uncertainties of stellar mass estimates via colour measurements}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1507.03016},
 keywords = {galaxies: clusters: individual: Virgo, galaxies: formation, galaxies: fundamental parameters, galaxies: general, galaxies: stellar content},
     year = 2015,
    month = sep,
   volume = 452,
    pages = {3209-3225},
      doi = {10.1093/mnras/stv1499},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.452.3209R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{DaCunha08,
   author = {{da Cunha}, E. and {Charlot}, S. and {Elbaz}, D.},
    title = "{A simple model to interpret the ultraviolet, optical and infrared emission from galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.1020},
 keywords = {dust, extinction , galaxies: ISM , galaxies: stellar content , infrared: galaxies},
     year = 2008,
    month = aug,
   volume = 388,
    pages = {1595-1617},
      doi = {10.1111/j.1365-2966.2008.13535.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.388.1595D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kalirai13,
   author = {{Kalirai}, J.~S. and {Anderson}, J. and {Dotter}, A. and {Richer}, H.~B. and 
	{Fahlman}, G.~G. and {Hansen}, B.~M.~S. and {Hurley}, J. and 
	{Reid}, I.~N. and {Rich}, R.~M. and {Shara}, M.~M.},
    title = "{Ultra-Deep Hubble Space Telescope Imaging of the Small Magellanic Cloud: The Initial Mass Function of Stars with M $\lt$\~{} 1 M $_{⊙}$}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1212.1159},
 keywords = {galaxies: photometry, galaxies: stellar content, Magellanic Clouds, methods: data analysis, methods: statistical, stars: luminosity function, mass function, techniques: photometric},
     year = 2013,
    month = feb,
   volume = 763,
      eid = {110},
    pages = {110},
      doi = {10.1088/0004-637X/763/2/110},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...763..110K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schodel09,
   author = {{Sch{\"o}del}, R. and {Merritt}, D. and {Eckart}, A.},
    title = "{The nuclear star cluster of the Milky Way: proper motions and mass}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0902.3892},
 keywords = {instrumentation: adaptive optics, techniques: high angular resolution, stars: kinematics, Galaxy: center, Galaxy: structure},
     year = 2009,
    month = jul,
   volume = 502,
    pages = {91-111},
      doi = {10.1051/0004-6361/200810922},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...502...91S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{McDermid15,
   author = {{McDermid}, R.~M. and {Alatalo}, K. and {Blitz}, L. and {Bournaud}, F. and 
	{Bureau}, M. and {Cappellari}, M. and {Crocker}, A.~F. and {Davies}, R.~L. and 
	{Davis}, T.~A. and {de Zeeuw}, P.~T. and {Duc}, P.-A. and {Emsellem}, E. and 
	{Khochfar}, S. and {Krajnovi{\'c}}, D. and {Kuntschner}, H. and 
	{Morganti}, R. and {Naab}, T. and {Oosterloo}, T. and {Sarzi}, M. and 
	{Scott}, N. and {Serra}, P. and {Weijmans}, A.-M. and {Young}, L.~M.
	},
    title = "{The ATLAS$^{3D}$ Project - XXX. Star formation histories and stellar population scaling relations of early-type galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1501.03723},
 keywords = {galaxies: abundances, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: stellar content},
     year = 2015,
    month = apr,
   volume = 448,
    pages = {3484-3513},
      doi = {10.1093/mnras/stv105},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.448.3484M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Merritt01a,
   author = {{Merritt}, D. and {Ferrarese}, L.},
    title = "{Black hole demographics from the M$_{•}$-{$\sigma$} relation}",
  journal = {\mnras},
   eprint = {astro-ph/0009076},
 keywords = {galaxies: active, galaxies: fundamental parameters, galaxies: kinematics and dynamics},
     year = 2001,
    month = jan,
   volume = 320,
    pages = {L30-L34},
      doi = {10.1046/j.1365-8711.2001.04165.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.320L..30M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Valluri05,
   author = {{Valluri}, M. and {Ferrarese}, L. and {Merritt}, D. and {Joseph}, C.~L.
	},
    title = "{The Low End of the Supermassive Black Hole Mass Function: Constraining the Mass of a Nuclear Black Hole in NGC 205 via Stellar Kinematics}",
  journal = {\apj},
   eprint = {astro-ph/0502493},
 keywords = {Galaxies: Elliptical and Lenticular, cD, Galaxies: Nuclei, Galaxies: Structure, Stellar Dynamics},
     year = 2005,
    month = jul,
   volume = 628,
    pages = {137-152},
      doi = {10.1086/430752},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...628..137V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gebhardt05,
   author = {{Gebhardt}, K. and {Rich}, R.~M. and {Ho}, L.~C.},
    title = "{An Intermediate-Mass Black Hole in the Globular Cluster G1: Improved Significance from New Keck and Hubble Space Telescope Observations}",
  journal = {\apj},
   eprint = {astro-ph/0508251},
 keywords = {Galaxies: Individual: Messier Number: M31, Galaxies: Star Clusters, Galaxy: Globular Clusters: General, globular clusters: individual (Mayall II ), globular clusters: individual ( G1)},
     year = 2005,
    month = dec,
   volume = 634,
    pages = {1093-1102},
      doi = {10.1086/497023},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634.1093G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Vandenbosch08,
   author = {{van den Bosch}, R.~C.~E. and {van de Ven}, G. and {Verolme}, E.~K. and 
	{Cappellari}, M. and {de Zeeuw}, P.~T.},
    title = "{Triaxial orbit based galaxy models with an application to the (apparent) decoupled core galaxy NGC 4365}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0712.0113},
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: kinematics and dynamics, galaxies: structure},
     year = 2008,
    month = apr,
   volume = 385,
    pages = {647-666},
      doi = {10.1111/j.1365-2966.2008.12874.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.385..647V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Merritt15,
   author = {{Merritt}, D.},
    title = "{Gravitational Encounters and the Evolution of Galactic Nuclei. IV. Captures Mediated by Gravitational-wave Energy Loss}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1511.08169},
 keywords = {black hole physics, galaxies: kinematics and dynamics, galaxies: nuclei},
     year = 2015,
    month = nov,
   volume = 814,
      eid = {57},
    pages = {57},
      doi = {10.1088/0004-637X/814/1/57},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...814...57M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barth06a,
   author = {{Barth}, A.~J. and {Darling}, J. and {Baker}, A.~J. and {Boizelle}, B.~D. and 
	{Buote}, D.~A. and {Ho}, L.~C. and {Walsh}, J.~L.},
    title = "{Toward Precision Black Hole Masses with ALMA: NGC 1332 as a Case Study in Molecular Disk Dynamics}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1603.04523},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160304523B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barth06b,
   author = {{Barth}, A.~J. and {Boizelle}, B.~D. and {Darling}, J. and {Baker}, A.~J. and 
	{Buote}, D.~A. and {Ho}, L.~C. and {Walsh}, J.~L.},
    title = "{Measurement of the Black Hole Mass in NGC 1332 from ALMA Observations at 0.044 Arcsecond Resolution}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1605.01346},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = may,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160501346B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fisher10,
   author = {{Fisher}, D.~B. and {Drory}, N.},
    title = "{Bulges of Nearby Galaxies with Spitzer: Scaling Relations in Pseudobulges and Classical Bulges}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1004.5393},
 keywords = {galaxies: bulges, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: structure},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {942-969},
      doi = {10.1088/0004-637X/716/2/942},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716..942F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Into&Laura13,
   author = {{Into}, T. and {Portinari}, L.},
    title = "{New colour-mass-to-light relations: the role of the asymptotic giant branch phase and of interstellar dust}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1301.2178},
 keywords = {stars: AGB and post-AGB, dust, extinction, galaxies: luminosity function, mass function, galaxies: stellar content, infrared: galaxies},
     year = 2013,
    month = apr,
   volume = 430,
    pages = {2715-2731},
      doi = {10.1093/mnras/stt071},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.430.2715I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McDonald11,
   author = {{McDonald}, M. and {Courteau}, S. and {Tully}, R.~B. and {Roediger}, J.
	},
    title = "{A survey of 286 Virgo cluster galaxies at optical griz and near-IR H band: surface brightness profiles and bulge-disc decompositions}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1105.0002},
 keywords = {surveys, galaxies: clusters: individual: Virgo, galaxies: fundamental parameters, galaxies: general, galaxies: photometry, galaxies: structure},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {2055-2068},
      doi = {10.1111/j.1365-2966.2011.18519.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.2055M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schodel14,
   author = {{Sch{\"o}del}, R. and {Feldmeier}, A. and {Kunneriath}, D. and 
	{Stolovy}, S. and {Neumayer}, N. and {Amaro-Seoane}, P. and 
	{Nishiyama}, S.},
    title = "{Surface brightness profile of the Milky Way's nuclear star cluster}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1403.6657},
 keywords = {dust, extinction, Galaxy: center, Galaxy: nucleus, Galaxy: structure, galaxies: nuclei, infrared: stars},
     year = 2014,
    month = jun,
   volume = 566,
      eid = {A47},
    pages = {A47},
      doi = {10.1051/0004-6361/201423481},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...566A..47S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Georgiev14,
   author = {{Georgiev}, I.~Y. and {B{\"o}ker}, T.},
    title = "{Nuclear star clusters in 228 spiral galaxies in the HST/WFPC2 archive: catalogue and comparison to other stellar systems}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1404.5956},
 keywords = {galaxies: spiral, galaxies: star clusters: general},
     year = 2014,
    month = jul,
   volume = 441,
    pages = {3570-3590},
      doi = {10.1093/mnras/stu797},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.441.3570G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Binney87,
   author = {{Binney}, J. and {Tremaine}, S.},
    title = "{Galactic dynamics}",
 keywords = {Astrophysics, Celestial Mechanics, Galactic Structure, Milky Way Galaxy, Dark Matter, Galactic Evolution, Jeans Theory, Orbital Mechanics, Potential Theory, Stellar Evolution, Stellar Systems},
    booktitle = "{Galactic dynamics}",
     year = 1987,
   adsurl = {http://adsabs.harvard.edu/abs/1987gady.book.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
  publisher = {Princeton University Press}
}

@ARTICLE{Laesker16,
   author = {{L{\"a}sker}, R. and {Greene}, J.~E. and {Seth}, A. and {van de Ven}, G. and 
	{Braatz}, J.~A. and {Henkel}, C. and {Lo}, K.~Y.},
    title = "{The Black Hole - Bulge Mass Relation in Megamaser Host Galaxies}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1602.06960},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160206960L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Onodera12,
   author = {{Onodera}, M. and {Renzini}, A. and {Carollo}, M. and {Cappellari}, M. and 
	{Mancini}, C. and {Strazzullo}, V. and {Daddi}, E. and {Arimoto}, N. and 
	{Gobat}, R. and {Yamada}, Y. and {McCracken}, H.~J. and {Ilbert}, O. and 
	{Capak}, P. and {Cimatti}, A. and {Giavalisco}, M. and {Koekemoer}, A.~M. and 
	{Kong}, X. and {Lilly}, S. and {Motohara}, K. and {Ohta}, K. and 
	{Sanders}, D.~B. and {Scoville}, N. and {Tamura}, N. and {Taniguchi}, Y.
	},
    title = "{Deep Near-infrared Spectroscopy of Passively Evolving Galaxies at z $\gt$\~{} 1.4}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1206.1540},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: high-redshift},
     year = 2012,
    month = aug,
   volume = 755,
      eid = {26},
    pages = {26},
      doi = {10.1088/0004-637X/755/1/26},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...755...26O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari16Rview,
   author = {{Cappellari}, M.},
    title = "{Structure and Kinematics of Early-Type Galaxies from Integral-Field Spectroscopy}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1602.04267},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160204267C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bresolin13,
   author = {{Bresolin}, F.},
    title = "{Clues on the Rejuvenation of the S0 Galaxy NGC 404 from the Chemical Abundance of Its Outer Disk}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1306.3027},
 keywords = {galaxies: abundances, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: individual: NGC 404, galaxies: ISM},
     year = 2013,
    month = aug,
   volume = 772,
      eid = {L23},
    pages = {L23},
      doi = {10.1088/2041-8205/772/2/L23},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...772L..23B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{McLaughlin15,
   author = {{McLaughlin}, D.~E. and {van der Marel}, R.~P.},
    title = "{Resolved Massive Star Clusters in the Milky Way and Its Satellites: Brightness Profiles and a Catalog of Fundamental Parameters}",
  journal = {\apjs},
   eprint = {astro-ph/0605132},
 keywords = {Galaxies: Star Clusters, Galaxy: Globular Clusters: General, Galaxies: Magellanic Clouds},
     year = 2005,
    month = dec,
   volume = 161,
    pages = {304-360},
      doi = {10.1086/497429},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJS..161..304M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari09,
   author = {{Cappellari}, M. and {Neumayer}, N. and {Reunanen}, J. and {van der Werf}, P.~P. and 
	{de Zeeuw}, P.~T. and {Rix}, H.-W.},
    title = "{The mass of the black hole in Centaurus A from SINFONI AO-assisted integral-field observations of stellar kinematics}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0812.1000},
 keywords = {black hole physics , instrumentation: adaptive optics , galaxies: elliptical and lenticular, cD , galaxies: individual: NGC 5128 , galaxies: kinematics and dynamics},
     year = 2009,
    month = apr,
   volume = 394,
    pages = {660-674},
      doi = {10.1111/j.1365-2966.2008.14377.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.394..660C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vanderMarel93,
   author = {{van der Marel}, R.~P. and {Franx}, M.},
    title = "{A new method for the identification of non-Gaussian line profiles in elliptical galaxies}",
  journal = {\apj},
 keywords = {Elliptical Galaxies, Galactic Structure, Line Spectra, Astronomical Models, Computational Astrophysics, Galactic Evolution},
     year = 1993,
    month = apr,
   volume = 407,
    pages = {525-539},
      doi = {10.1086/172534},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...407..525V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bartko10,
   author = {{Bartko}, H. and {Martins}, F. and {Trippe}, S. and {Fritz}, T.~K. and 
	{Genzel}, R. and {Ott}, T. and {Eisenhauer}, F. and {Gillessen}, S. and 
	{Paumard}, T. and {Alexander}, T. and {Dodds-Eden}, K. and {Gerhard}, O. and 
	{Levin}, Y. and {Mascetti}, L. and {Nayakshin}, S. and {Perets}, H.~B. and 
	{Perrin}, G. and {Pfuhl}, O. and {Reid}, M.~J. and {Rouan}, D. and 
	{Zilka}, M. and {Sternberg}, A.},
    title = "{An Extremely Top-Heavy Initial Mass Function in the Galactic Center Stellar Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0908.2177},
 keywords = {Galaxy: center, stars: early-type, stars: luminosity function, mass function},
     year = 2010,
    month = jan,
   volume = 708,
    pages = {834-840},
      doi = {10.1088/0004-637X/708/1/834},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...708..834B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lu.R13,
   author = {{Lu}, J.~R. and {Do}, T. and {Ghez}, A.~M. and {Morris}, M.~R. and 
	{Yelda}, S. and {Matthews}, K.},
    title = "{Stellar Populations in the Central 0.5 pc of the Galaxy. II. The Initial Mass Function}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1301.0540},
 primaryClass = "astro-ph.SR",
 keywords = {Galaxy: center, infrared: stars, methods: statistical, stars: evolution, stars: luminosity function, mass function, stars: massive},
     year = 2013,
    month = feb,
   volume = 764,
      eid = {155},
    pages = {155},
      doi = {10.1088/0004-637X/764/2/155},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...764..155L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Martin-Navarro15,
   author = {{Mart{\'{\i}}n-Navarro}, I. and {Barbera}, F.~L. and {Vazdekis}, A. and 
	{Falc{\'o}n-Barroso}, J. and {Ferreras}, I.},
    title = "{Radial variations in the stellar initial mass function of early-type galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1404.6533},
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters},
     year = 2015,
    month = feb,
   volume = 447,
    pages = {1033-1048},
      doi = {10.1093/mnras/stu2480},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.447.1033M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{VandenBosch16a,
   author = {{van den Bosch}, R.},
    title = "{Unification of the Fundamental Plane and Super-Massive Black Holes Masses}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1606.01246},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160601246V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Walsh16,
   author = {{Walsh}, J.~L. and {van den Bosch}, R.~C.~E. and {Gebhardt}, K. and 
	{Y{\i}ld{\i}r{\i}m}, A. and {Richstone}, D.~O. and {G{\"u}ltekin}, K. and 
	{Husemann}, B.},
    title = "{A 5 x 10$^{9}$ Msun Black Hole in NGC 1277 from Adaptive Optics Spectroscopy}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1511.04455},
 keywords = {black hole physics, galaxies: elliptical and lenticular, cD, galaxies: individual: NGC 1277, galaxies: kinematics and dynamics, galaxies: nuclei},
     year = 2016,
    month = jan,
   volume = 817,
      eid = {2},
    pages = {2},
      doi = {10.3847/0004-637X/817/1/2},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...817....2W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Thater16,
   author = {{Thater}, S. and {Krajnovi{\'c}}, D. and {Bourne}, M.~A. and 
	{Cappellari}, M. and {de Zeeuw}, T. and {Emsellem}, E. and {Magorrian}, J. and 
	{McDermid}, R.~M. and {Sarzi}, M. and {van de Ven}, G.},
    title = "{A low upper mass limit for the central black hole in the late-type galaxy NGC 4414}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1610.04269},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161004269T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
